Data-centric Dynamic Partial Order Reduction

We present a new dynamic partial-order reduction method for stateless model checking of concurrent programs. A common approach for exploring program behaviors relies on enumerating the traces of the program, without storing the visited states (aka stateless exploration). As the number of distinct traces grows exponentially, dynamic partial-order reduction (DPOR) techniques have been successfully used to partition the space of traces into equivalence classes (Mazurkiewicz partitioning), with the goal of exploring only few representative traces from each class. We introduce a new equivalence on traces under sequential consistency semantics, which we call the observation equivalence. Two traces are observationally equivalent if every read event observes the same write event in both traces. While the traditional Mazurkiewicz equivalence is control-centric, our new definition is data-centric. We show that our observation equivalence is coarser than the Mazurkiewicz equivalence, and in many cases even exponentially coarser. We devise a DPOR exploration of the trace space, called data-centric DPOR, based on the observation equivalence. For acyclic architectures, our algorithm is guaranteed to explore exactly one representative trace from each observation class, while spending polynomial time per class. Hence, our algorithm is optimal wrt the observation equivalence, and in several cases explores exponentially fewer traces than any enumerative method based on the Mazurkiewicz equivalence. For cyclic architectures, we consider an equivalence between traces which is finer than the observation equivalence; but coarser than the Mazurkiewicz equivalence, and in some cases is exponentially coarser. Our data-centric DPOR algorithm remains optimal under this trace equivalence.

==> annotations_bk.tex <==
\section{Annotations}\label{sec:annotations}
%\vspace{-0.5em}

In this section we introduce the notion of \emph{annotations}, which are 
intended constraints on the observation functions that traces discovered by 
our data-centric DPOR ($\EnumExplore$) are required to meet.
%We show that in the general case, constructing a trace that satisfies an annotation is \NPC.
%However, over acyclic architectures the problem can be solved in polynomial time (in fact, cubic time in the size of the constructed trace).
%In \cref{sec:cyclic_architectures} we extend the algorithms of this section to cyclic architectures.

\noindent{\bf Annotations.}
An \emph{annotation pair} $\Annotation=(\Annotationpos, \Annotationneg)$ is a pair of
\begin{compactenum}
\item a \emph{positive annotation} $\Annotationpos: \SysReads \pto \SysWrites$, and
\item a \emph{negative annotation} $\Annotationneg: \SysReads \pto 2^{\SysWrites}$
\end{compactenum}
such that for all read events $\Read$, if $\Annotationpos(\Read)=\Write$, then we have $\Confl(\Read, \Write)$ and it is not the case that $\PS(\Read, \Write)$.
We will use annotations to guide the recursive calls of $\EnumExplore$ towards traces that belong to different equivalence classes
than the ones explored already, or will be explored by other branches of the algorithm.
A positive annotation $\Annotationpos$ forces $\EnumExplore$ to explore traces that are compatible with $\Annotationpos$
(or abort the search if no such trace can be generated).
Since a positive annotation is an ``intended'' observation function, we say that a trace $\Trace$ \emph{realizes} $\Annotationpos$ if $\Obs_{\Trace}=\Annotationpos$, in which case $\Annotationpos$ is called \emph{realizable}.
A negative annotation $\Annotationneg$ prevents $\EnumExplore$ from exploring traces $\Trace$ in which a read event observes a write event that belongs to its negative annotation set (i.e., $\Obs_{\Trace}(\Read)\in \Annotationneg(\Read)$).
%\noindent{\em Only positive annotations.}
In the remaining section we focus on positive annotations, and the problem of deciding whether a positive annotation is realizable.
%Negative annotations will become useful in the next section, where they will be used together with positive annotations to guide 
%the data-centric DPOR.



\noindent{\bf The value function $\Value_{\Annotationpos}$.}
Given a positive annotation $\Annotationpos$, we define the relation $<_{\Annotationpos}\subseteq \Image(\Annotationpos)\times \Domain(\Annotationpos)$ such that $\Write <_{\Annotationpos} \Read$ iff $(\Read, \Write)\in \Annotationpos$.
The positive annotation $\Annotationpos$ is \emph{acyclic} if the relation $\PS \cup <_{\Annotationpos}$ is a strict partial order (i.e., it contains no cycles).
The \emph{value function} $\Value_{\Annotationpos}:\Domain(\Annotationpos)\cup \Image(\Annotationpos)\to \ValueDomain$ of an acyclic positive annotation $\Annotationpos$ is the unique function defined inductively, as follows.
\begin{compactenum}
\item For each $\Write\in\Image(\Annotationpos)$ of the form $\Write:g\gets \mathsf{write}~f(v_1,\dots,v_{n_i})$, we have $\Value_{\Annotationpos}(\Write)=f(\alpha_1,\dots, \alpha_{n_i})$, where for each $\alpha_j$ we have
\begin{compactenum}
\item $\alpha_j=\Value_{\Annotationpos}(\Read)$ if there exists a read event $\Read\in \Domain(\Annotationpos)$ 
such that (i)~$\Read$ is of the form $\Read: v_j\gets \mathsf{read}~g'$ and (ii)~$\PS(\Read, \Write)$ and (iii)~there exists no other $\Read'\in \Domain(\Annotationpos)$ with $\PS(\Read, \Read')$ and which satisfies conditions (i)~and (ii).
\item $\alpha_j$ equals the initial value of $v_i$ otherwise.
\end{compactenum}
\item For each $\Read\in \Domain(\Annotationpos)$ we have $\Value_{\Annotationpos}(\Read)= \Value_{\Annotationpos}(\Annotationpos(\Read))$.
\end{compactenum}
Note that $\Value_{\Annotationpos}$ is well-defined, as for any read event $\Read$ that is used to define the value of a write event $\Write$ we have $\PS(\Read, \Write)$, and thus by the acyclicity of $\Annotationpos$, $\Value_{\Annotationpos}(\Read)$ does not depend on $\Value_{\Annotationpos}(\Write)$.


\begin{comment}
\noindent{\bf The value function $\Value_{\Annotationpos}$.}
Given a positive annotation $\Annotationpos$, we define the relation $<_{\Annotationpos}\subseteq \Image(\Annotationpos)\times \Domain(\Annotationpos)$ such that $\Write <_{\Annotationpos} \Read$ iff $(\Read, \Write)\in \Annotationpos$.
The positive annotation $\Annotationpos$ is \emph{acyclic} if the relation $\PS \cup <_{\Annotationpos}$ is a strict partial order (i.e., it contains no cycles).
We let $\bot\in \ValueDomain$ be a distinguished value of the domain of the program variables.
The \emph{value function} $\Value_{\Annotationpos}:\Domain(\Annotationpos)\cup \Image(\Annotationpos)\to \ValueDomain^{\bot}$ of an acyclic positive annotation $\Annotationpos$ is the unique function defined inductively, as follows.
\begin{compactenum}
\item For each $\Write\in\Image(\Annotationpos)$ of the form $\Write:g\gets \mathsf{write}~f(v_1,\dots,v_{n_i})$,
we define $\alpha_j$, for $1\leq j\leq n_i$, as follows.
\begin{compactenum}
\item If $v_j$ is a constant, then $\alpha_j=v_j$.
\item If $v_j$ is a variable, 
\end{compactenum}
Finally, we define $\Value_{\Annotationpos}(\Write)=f(\alpha_1,\dots, \alpha_{n_i})$ if $\alpha_j\neq \bot$ for all $j$, and $\Value_{\Annotationpos}(\Write)=\bot$ otherwise.

we have $\Value_{\Annotationpos}(\Write)=f(\alpha_1,\dots, \alpha_{n_i})$, where for each $\alpha_j$ we have
\begin{compactenum}
\item $\alpha_j=\Value_{\Annotationpos}(\Read)$ if there exists a read event $\Read\in \Domain(\Annotationpos)$ 
such that (i)~$\Read$ is of the form $\Read: v_j\gets \mathsf{read}~g'$ and (ii)~$\PS(\Read, \Write)$ and (iii)~there exists no other $\Read'\in \Domain(\Annotationpos)$ with $\PS(\Read, \Read')$ and which satisfies conditions (i)~and (ii).
\item $\alpha_j$ equals the initial value of $v_i$ otherwise.
\end{compactenum}
\item For each $\Read\in \Domain(\Annotationpos)$ we have $\Value_{\Annotationpos}(\Read)= \Value_{\Annotationpos}(\Annotationpos(\Read))$.
\end{compactenum}

\end{comment}

%\begin{compactenum}
%\item For each $\Write\in\Image(\Annotationpos)$ of the form $\Write:g\gets \mathsf{write}~f(v_1,\dots,v_{n_i})$, we have $\Value_{\Annotationpos}(\Write)=f(\alpha_1,\dots, \alpha_{n_i})$, where for each $\alpha_j$ we have
%\begin{compactenum}
%\item $\alpha_j=\Value_{\Annotationpos}(\Read)$ if there exists a read event $\Read\in \Domain(\Annotationpos)$ 
%such that (i)~$\Read$ is of the form $\Read: v_j\gets \mathsf{read}~g'$ and (ii)~$\PS(\Read, \Write)$ and (iii)~there exists no other $\Read'\in \Domain(\Annotationpos)$ with $\PS(\Read, \Read')$ and which satisfies conditions (i)~and (ii).
%\item $\alpha_j$ equals the initial value of $v_i$ otherwise.
%\end{compactenum}
%\item For each $\Read\in \Domain(\Annotationpos)$ we have $\Value_{\Annotationpos}(\Read)= \Value_{\Annotationpos}(\Annotationpos(\Read))$.
%\end{compactenum}


\begin{remark}\label{rem:annotationpos_value}
If $\Annotationpos$ is realizable then it is acyclic,
and for any trace $\Trace$ that realizes $\Annotationpos$ we have that $\Value_{\Trace}=\Value_{\Annotationpos}$.
\end{remark}

\noindent{\bf Well-formed annotations and basis of annotations.}
A positive annotation $\Annotationpos$ is called \emph{well-formed} if the following conditions hold:
\begin{compactenum}
\item\label{item:acyclicity} $\Annotationpos$ is acyclic.
\item\label{item:lock_obs} For every lock-release event $\Event_{a}\in \Image(\Annotationpos)\cap \SysAcquires$
there is at most one lock-acquire event $\Event_{r}\cap \SysReleases$ such that $\Annotationpos(\Event_{a})=\Event_{r}$.
\item\label{item:basis} There exist sequential traces $(\SeqTrace_i)_i$, one for each process $\Process_i$, such that each $\SeqTrace_i$ ends in a global event, and the following conditions hold. 
\begin{compactenum}
\item for every pair of lock-acquire events $\Event_a^1, \Event_a^2\in \Events{\SeqTrace_i}\cap \SysAcquires$ such that $\Index_{\SeqTrace_i}(\Event_a^1)<\Index_{\SeqTrace_i}(\Event_a^2)$ and $\Location(\Event_a^1)=\Location(\Event_a^2)$
there exists a lock release event $\Event_r\in \Events{\SeqTrace_i}\cap \SysReleases$ such that 
$\Index_{\SeqTrace_i}(\Event_a^1)<\Index{\SeqTrace_i}(\Event_r)< \Index{\SeqTrace_i}(\Event_a^2)$ and $\Location(\Event_r)=\Location(\Event_a^1)=\Location(\Event_a^2)$.
\item $\bigcup_i \Reads{\SeqTrace_i} = \Domain(\Annotationpos)$ and $\Image(\Annotationpos) \subseteq \bigcup_i \Writes{\SeqTrace_i}$,
i.e., $(\SeqTrace_i)_i$ contains precisely the read events of $\Annotationpos$ and a superset of the write events.
\item Each $\SeqTrace_i$ corresponds to a deterministic computation of process $\Process_i$, where the value of every global event $\Event$ during the computation is taken to be $\Value_{\Annotationpos}(\Event)$.
%Because of Item~1, this is well-defined.
\end{compactenum}
\end{compactenum}

The sequential traces $(\SeqTrace_i)_i$ are called a \emph{basis} of $\Annotationpos$ if every $\SeqTrace_i$ is minimal in length.
The following lemma establishes properties of well-formedness and basis.

\begin{comment}
\begin{compactenum}
\item 
\begin{compactenum}
\item for every lock-acquire event $\Event_a\in \Events{\SeqTrace_i}$ there exists a lock-release event $\Event_r\in \Events{\Trace}$ such that $\Location(\Event_a)=\Location(\Event_r)$ and $\Index_{\SeqTrace_i}(\Event_a)< \Index_{\SeqTrace}(\Event_r)$, and
\item for every pair of lock-acquire events $\Event_a^1, \Event_a^2\in \Events{\SeqTrace_i}\cap \SysAcquires$ such that $\Index{\SeqTrace_i}(\Event_a^1)<\Index_{\SeqTrace_i}(\Event_a^2)$ and $\Location(\Event_a^1)=\Location(\Event_a^2)$
there exists a lock release event $\Event_r\in \Events{\SeqTrace_i}\cap \SysReleases$ such that 
$\Index_{\SeqTrace_i}(\Event_a^1)<\Index{\SeqTrace_i}(\Event_r)< \Index{\SeqTrace_i}(\Event_a^2)$ and $\Location(\Event_r)=\Location(\Event_a^1)=\Location(\Event_a^2)$.
\end{compactenum}
\item $\bigcup_i \Reads{\SeqTrace_i} = \Domain(\Annotationpos)$ and $\bigcup_i \Writes{\SeqTrace_i}\subseteq \Image(\Annotationpos)$,
i.e., $(\SeqTrace_i)_i$ contains precisely the read events of $\Annotationpos$ and a superset of the write events.
\item Each $\SeqTrace_i$ corresponds to a deterministic computation of process $\Process_i$, where the value of every global event $\Event$ during the computation is taken to be $\Value_{\Annotationpos}(\Event)$.
%Because of Item~1, this is well-defined.
\end{compactenum}
The sequential traces $(\SeqTrace_i)_i$ are called a \emph{basis} of $\Annotationpos$ if every $\SeqTrace_i$ is minimal in length.
The following lemma establishes properties of well-formedness and basis.
\end{comment}


\begin{restatable}{lemma}{annotationbasis}
\label{lem:annotation_basis}
Let $X=\Domain(\Annotationpos)\cup \Image(\Annotationpos)$ be the set of events that appear in a positive annotation $\Annotationpos$, and $X_i=X\cap \SysEvents_i$ the subset of events of $X$ from process $\Process_i$.
The following assertions hold:
\begin{compactenum}
\item If $\Annotationpos$ is well-formed, then it has a unique basis $(\SeqTrace_i)_i$.

\item Computing the basis of $\Annotationpos$ (or concluding that $\Annotationpos$ is not well-formed)
can be done in $O(n)$ time, where $n=\sum_i(|\SeqTrace_i|)$
if $\Annotationpos$ is well-formed, otherwise $n= \sum_i \ell_i$,
where $\ell_i$ is the length of the longest path from the root $\Root_i$ of $\CFG_i$ to an event $\Event\in X_i$.

\item For every trace $\Trace$ that realizes $\Annotationpos$ we have that 
$\Annotationpos$ is well-formed and $\Trace\in \SeqTrace_1 \Conv \dots \Conv \SeqTrace_k$.
\end{compactenum}
\end{restatable}


%
%\begin{lemma}\label{lem:annotation_basis}
%Let $X=\Domain(\Annotationpos)\cap \Image(\Annotationpos)$ be the set of events that appear in a positive annotation $\Annotationpos$, and $X_i=X\cap \SysEvents_i$ the subset of events of $X$ from process $\Process_i$.
%The following assertions hold:
%\begin{compactitem}
%\item If $\Annotationpos$ is well-formed, then it has a unique basis $(\SeqTrace_i)_i$.
%
%\item Computing the basis of $\Annotationpos$ (or concluding that $\Annotationpos$ is not well-formed)
%can be done in $O(n)$ time, where $n=\sum_i(|\SeqTrace_i|)$
%if $\Annotationpos$ is well-formed, otherwise $n= \sum_i \ell_i$,
%where $\ell_i$ is the length of the longest path from the root $\Root_i$ of $\CFG_i$ to an event $\Event\in X_i$.
%
%\item For every trace $\Trace$ that realizes $\Annotationpos$ we have that 
%$\Annotationpos$ is well-formed and $\Trace\in \SeqTrace_1 \Conv \dots \Conv \SeqTrace_k$.
%\end{compactitem}
%\end{lemma}




%\vspace{-1em}
\subsection{The Hardness of Realizing Positive Annotations}\label{subsec:get_trace}
%\vspace{-0.5em}

A core step in our data-centric DPOR algorithm is constructing a trace that realizes a positive annotation.
That is, given a positive annotation $\Annotationpos$, the goal is to obtain a trace $\Trace$ (if one exists) such that
$\Obs_{\Trace}=\Annotationpos$, i.e., $\Trace$ contains precisely the read events of $\Annotationpos$,
and every read event in $\Trace$ observes the write event specified by $\Annotationpos$.
Here, we show that the problem is \NPC~in the general case.
Membership in \NP~is trivial, since, given a trace $\Trace$, it is straightforward to verify that $\Obs_{\Trace}=\Annotationpos$ in $O(|\Trace|)$ time.
Hence our focus will be on establishing \NP-hardness.
For doing so, we introduce a new graph problem, namely \AEA, which is closely related to the problem of realizing a positive annotation under sequential consistency semantics.
We first show that \AEA~is \NPH, and afterwards that the problem is polynomial-time reducible to realizing a positive annotation.


\noindent{\bf The problem \AEA.}
The input to the problem is a pair $(G,H)$ where $G=(V,E)$ is a directed acyclic graph, and $H=\{(x_i,y_i, z_i)\}_i$ is a set of triplets of distinct nodes such that
\begin{compactenum}
\item $x_i,y_i,z_i\in V$, $(y_i,z_i)\in E$ and $(x_i,y_i), (z_i, x_i)\not \in E$, and
\item each node $x_i$ and $y_i$ appears only once in $H$.
\end{compactenum}
An \emph{edge addition set} $X=\{e_i\}_{i=1}^{|H|}$ for $(G,H)$ is a set of edges $e_i\in E$ such that for each $e_i$ we have either $e_i=(x_i,y_i)$ or $e_i=(z_i,x_i)$.
The problem \AEA~asks whether there exists an edge addition set $X$ for $(G,H)$ such that the graph $G_X=(V, E\cup X)$ remains acyclic.



\begin{restatable}{lemma}{aea}
\label{lem:aea}
\AEA~is \NPH.
\end{restatable}
\noindent{\em Sketch.}
The proof is by reduction from \SATMONOTONE~\cite[LO4]{Garey79}.
In \SATMONOTONE, the input is a propositional 3CNF formula $\phi$ in which every literal is positive,
and the goal is to decide whether there exists a satisfying assignment for $\phi$ that assigns exactly one literal per clause to $\True$.
The reduction proceeds as follows.
In the following, we let $C$ and $D$ range over the clauses and $x_i$ over the variables of $\phi$.
We assume w.l.o.g. that no variable repeats in the same clause.
For every variable $x_i$, we introduce a node $\Write'_i\in V$.
For every clause $C=(x_{C_1}\lor x_{C_2} \lor x_{C_3})$, we introduce a pair of nodes $\Write^C_{C_j}, \Read^C_{C_j}\in V$
and an edge $(\Write^C_{C_j}, \Read^C_{C_j})\in E$, where $j\in \{1,2,3\}$.
Additionally, we introduce an edge $(\Write^C_{C_j}, \Write'_{C_l})\in E$ for every pair $j,l\in\{1,2,3\}$ such that $j\neq l$,
and an edge $(\Write'_{C_j}, \Read^C_{C_l})$ for each $j\in \{1,2,3\}$, where $l=( j+1) \mod 3 + 1$.
Finally, for every pair of clauses $C, D$ and $l_1,l_2\in \{1,2,3\}$ such that $C_{l_1}=D_{l_2}=\ell$
(i.e., $C$ and $D$ share the same variable $x_{\ell}$ in positions $l_1$ and $l_2$),
we add edges $(\Write^{C}_{\ell}, \Read^{D}_{\ell}), (\Write^{D}_{\ell}, \Read^{C}_{\ell})\in E$.
The set $H$ consists of triplets of nodes $(\Write'_{C_j},\Write^C_{C_j},\Read^C_{C_j})$ for every clause $C$ and $j\in\{1,2,3\}$.
Figure~\ref{fig:reduction} illustrates the construction.



\input{fig_reduction}


\noindent{\bf From \AEA~ to annotations.}
Finally, we argue that \AEA~is polynomial-time reducible to realizing a positive annotation.
Given an instance $(G,H)$ of \AEA, with $G=(V,E)$, we construct an architecture $\System$ of $k=2\cdot |H|$ processes $(\Process_i)_i$, and a positive annotation $\Annotationpos$.
We assume, w.l.o.g., that the set of nodes $V$ is precisely the set of nodes that appear in the triplets of $H$.
Indeed, any other nodes can be removed while maintaining the connectivity between the nodes in the triplets of $H$,
and any edge addition set $X$ solves the problem in the original graph iff it does so in the reduced graph.
The construction proceeds in two steps.
\begin{compactenum}
\item For every triplet $(x_i, y_i, z_i)\in H$, we create two events $\Write_{i}\in \SysWrites$, $\Read_{i}\in \SysReads$ in $\Process_i$ such that $\PS(\Write_i, \Read_i)$, and an event $\Write'_{i}$ in process $\Process_{|H|+i}$. For all three events we set $\Location(\Read_i)=\Location(\Write_i)=\Location(\Write'_i)=g_i$, where $g_i\in \Globals$ is some fresh global variable of $\System$.
Finally, we introduce $(\Read_i, \Write_i)\in \Annotationpos$.
Given any node $u\in V$, let $\Event(u)$ denote the event associated with $u$.
\item For every edge $(u,v)$ we introduce a new global variable $g\in \Globals$, and two events $\Write_{u,v}\in \SysWrites$, $\Read_{u,v}\in \SysReads$ such that $\Location(\Write_{u,v})=\Location(\Read_{u,v})=g$.
We make $\Write_{u,v}$ an event of the same process as $\Event(u)$, and $\Read_{u,v}$ an event of the same process as $\Event(v)$,
and additionally $\PS(\Event(u), \Write_{u,v})$ and $\PS(\Read_{u,v}, \Event(v))$.
Finally, we introduce $(\Read_{u,v}, \Write_{u,v})\in \Annotationpos$.
\end{compactenum}

Observe that the above construction is linear in the size of $(G, H)$.
The following lemma states the correctness of the reduction. 


\begin{restatable}{lemma}{aatoann}
\label{lem:aatoann}
The decision problem of \AEA~on input $(G=(V,E),H)$ admits a positive answer iff the positive annotation $\Annotationpos$ is realizable in $\System$.
\end{restatable}
%The following lemma states the correctness of the reduction.
%
%\begin{restatable}{lemma}{aatoann}
%\label{lem:aatoann}
%The decision problem of \AEA~on input $(G=(V,E),H)$ admits a positive answer iff the positive annotation $\Annotationpos$ is realizable in $\System$.
%\end{restatable}



%\vspace{-1em}
\subsection{Realizing Positive Annotations in Acyclic Architectures}
%\vspace{-0.5em}

We now turn our attention to a tractable fragment of the positive annotation problem.
Here we show that if $\System$ is an acyclic architecture, then the problem admits a polynomial-time solution
(in fact, cubic in the size of the constructed trace).
%We present a procedure $\Realize$, which takes as input a positive annotation $\Annotationpos$ and an acyclic architecture $\System$,
%and constructs a trace $\Trace$ that realizes $\Annotationpos$ (or concludes that $\Annotationpos$ is not realizable).

\noindent{\bf Intuition.}
The hardness of realizing positive annotations in general architectures comes from transitivity constraints that 
ensure that the resulting happens-before relation is acyclic. 
That is, for every triplet of events $\Event_1, \Event_2, \Event_3$,  deciding that (i)~$\Event_1$ happens before $\Event_2$ and (ii)~$\Event_2$ happens before $\Event_3$ must lead in (iii)~$\Event_1$ happening before $\Event_3$.
In general architectures, such a triplet of events is, in general, \emph{unrelated a-priori}, and hence an algorithm that constructs a trace out of a positive annotation need to make the above decisions (i)-(iii) consistently.
In contrast, acyclic architectures have the property that in every such triplet of events, a pair of them always belongs to the same process and thus is \emph{ordered a-priori} by the program structure. This allows to express transitivity constraints by means of a 2SAT encoding.
For example assume that $\Event_2,\Event_3$ belong to the same process and $\Event_2$ is ordered before $\Event_3$ by the program structure.
Then the transitivity constraints can be simply encoded in a 2SAT clause 
$(x_{\Event_1, \Event_2}\Rightarrow x_{\Event_1, \Event_3})$, 
where $x_{\Event, \Event'}$ is interpreted as a boolean variable indicating that $\Event$ happens before $\Event'$.
Besides transitivity constraints, observe that positive annotation constraints can also be encoded in a 2SAT clause.
That is, every positive annotation constraint $\Annotationpos(\Read)=\Write$ can be encoded in a 2SAT clause 
$(x_{\Write', \Read} \Rightarrow x_{\Write', \Write})$, 
for every write event $\Write'\neq \Write$ that conflicts with $\Write$.

\noindent{\bf Procedure $\Realize$.}
Let $\System$ be an acyclic architecture, and $\Annotationpos$ a positive annotation over $\System$.
We describe a procedure $\Realize(\Annotationpos)$ which returns a trace $\Trace$ that realizes $\Annotationpos$, or $\bot$ if $\Annotationpos$ is not realizable.
The procedure works in two phases.
In the first phase, $\Realize(\Annotationpos)$ uses Lemma~\ref{lem:annotation_basis} to extract a basis $(\SeqTrace_i)_i$ of $\Annotationpos$.
In the second phase, $\Realize(\Annotationpos)$ determines whether the events of $\bigcup_i \Events{\SeqTrace_i}$ can be linearized in a trace $\Trace$ such that $\Obs_{\Trace}=\Annotationpos$.
Informally, the second phase consists of constructing a 2SAT instance over variables $x_{\Event_1,\Event_2}$, where $\Event_1,\Event_2\in \bigcup_i\Events{\SeqTrace_i}$.
Setting $x_{\Event_1,\Event_2}$ to $\True$ corresponds to making $\Event_1$ happen before $\Event_2$ in the witness trace $\Trace$.
The clauses of the 2SAT instance capture four properties that each such ordering needs to meet, namely that
\begin{compactenum}
\item the resulting assignment produces a total order (totality, antisymmetry and transitivity) between all of the events that appear in adjacent processes in the communication graph $G_{\System}$,
\item the produced total order respects the positive annotation, i.e., every write event $\Write'$ that conflicts with an annotated read/write pair $(\Read,\Write)\in \Annotationpos$ must either happen before $\Write$ or after $\Read$, and
%\item the produced total order respects the lock semantics, i.e., between every two lock-acquire events on the same lock there must be a lock-release event, and
\item the produced total order respects the partial order induced by the program structure $\PS$ and the positive annotation $\Annotationpos$.
\end{compactenum}


\newsavebox{\constructgraph}
\begin{algorithm}
\small
%\renewcommand{\thealgocf}{}
%\SetAlgorithmName{Benchmark}{algorithm}
\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\Realize(\Annotationpos)$}\label{algo:realize}
\KwIn{A positive annotation $\Annotationpos$ with basis $(\SeqTrace_i)_i$ }
\KwOut{A trace $\Trace$ that realizes $\Annotationpos$ or $\bot$ if $\Annotationpos$ is not realizable}
\BlankLine
Construct a directed graph $G=(V,E)$ where\label{line:graph_G}\\
\Indp
- $V=\bigcup_i \Events{\SeqTrace_i}$, and\\
- $E=\{(\Event_1, \Event_2):~  (\Event_2,\Event_1)\in \Annotationpos \text{ ~or~ } \PS(\Event_1,\Event_2) \}$\\
\Indm
$G^*=(V, E^*)\gets$ the transitive closure of $G$\label{line:closure}\\
\tcp{A set $\mathcal{C}$ of 2SAT clauses over variables $V_\mathcal{C}$}
$\mathcal{C}\gets \emptyset$\\
$V_{\mathcal{C}}\gets \{x_{\Event_1, \Event_2}:~\Event_1, \Event_2\in V \text{ and } \Event_1\neq \Event_2 \text{ and either } \Proc(\Event_1)=\Proc(\Event_2) \text{ or } (\Proc(\Event_1), \Proc(\Event_2))\in E_{\System} \}$\label{line:variables}\\
\tcp{1.~Antisymmetry clauses}
\ForEach{$x_{\Event_1, \Event_2} \in V_{\mathcal{C}}$}{\label{line:antisymmetry}
$\mathcal{C}\gets \mathcal{C} \cup \{ (x_{\Event_1,\Event_2}\Rightarrow \neg x_{\Event_2, \Event_1}), (\neg x_{\Event_2, \Event_1} \Rightarrow x_{\Event_1, \Event_2}) \}$
}
\tcp{2.~Transitivity clauses}
\ForEach{$x_{\Event_1, \Event_2} \in V_{\mathcal{C}}$}{\label{line:transitivity}
\ForEach{$(\Event_2,\Event_3)\in E^*$}{
$\mathcal{C}\gets \mathcal{C} \cup \{ (x_{\Event_1, \Event_2} \Rightarrow x_{\Event_1, \Event_3})\}$
}
\ForEach{$(\Event_3, \Event_1)\in E^*$}{
$\mathcal{C}\gets \mathcal{C} \cup \{ (x_{\Event_1, \Event_2} \Rightarrow x_{\Event_3, \Event_2})\}$
}
}
\tcp{3.~Annotation clauses}
\ForEach{$(\Read, \Write)\in \Annotationpos$ and $\Write'\in V\cap \SysWrites$ s.t. $\Confl(\Read, \Write')$}{\label{line:annotation}
%$\mathcal{C}\gets \mathcal{C} \cup \{ (x_{\Write', \Read} \Rightarrow x_{\Write', \Write}), (x_{\Write, \Write'} \Rightarrow x_{\Read, \Write'})  \}$
$\mathcal{C}\gets \mathcal{C} \cup \{ (x_{\Write', \Read} \Rightarrow x_{\Write', \Write})\}$
}
\tcp{4.~Fact clauses}
\ForEach{$(\Event_1, \Event_2)\in E^*$ with $\Event_1\neq \Event_2$}{\label{line:fact}
$\mathcal{C}\gets \mathcal{C} \cup \{(x_{\Event_1, \Event_2})\}$
}
Compute a satisfying assignment $f:V_{\mathcal{C}}\to \{\False, \True\}^{|V_{\mathcal{C}}|}$ of 
the 2SAT over $\mathcal{C}$, or \Return $\bot$ if $\mathcal{C}$ is unsatisfiable\label{line:2SAT}\\
$E'\gets E \cup \{(\Event_1, \Event_2):~f(x_{\Event_1, \Event_2})=\True\}$\\
Let $G'=(V,E')$\label{line:topological_order}\\
\Return a trace $\Trace$ by topologically sorting the vertices of $G'$\label{line:return_trace}
\end{algorithm}


The formal description of the second phase is given in Algorithm~\ref{algo:realize}.
The following theorem summarizes the results of this section.


\begin{restatable}{theorem}{annotation}\label{them:annotation}
Consider any architecture $\System=(\Process)_i$ and let $\Annotationpos$ be any well-formed positive annotation over a basis $(\SeqTrace)_i$.
Deciding whether $\Annotationpos$ is realizable is \NPC.
If $\System$ is acyclic, the problem can be solved in $O(n^3)$ time, where $n=\sum_i|\SeqTrace_i|$.
\end{restatable}


==> benchmarks.tex <==
\section{Benchmarks}\label{sec:benchmarks}

The following provides the pseudocode for the two synthetic benchmarks \emph{lastzero} (taken from~\cite{Abdulla14}) and \emph{opt\_lock},
found in Section~\ref{subsec:experiments}.

\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\small
\SetKwInOut{Globals}{Globals}
\SetKwInOut{Locals}{Locals}
\setcounter{algocf}{-1}
\renewcommand{\thealgocf}{}
\SetAlgorithmName{Benchmark}{algorithm}
\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{\emph{lastzero}($n$), for $n+1$ processes}
\Globals{
$\mathit{int}~\mathsf{array}[n+1]$\\
}
\BlankLine
\tcp{--------- Process $j=0$ ---------}
\Locals{$\mathit{int}~i$}
$i\gets n$\\
\While{$\mathsf{array}[i]\neq 0$}{
$i\gets i-1$
}
\BlankLine
\BlankLine
\BlankLine
\tcp{--------- Process $1< j\leq n$ ---------}
%\BlankLine
$\mathsf{array}[j]\gets \mathsf{array}[j-1] + 1$
\BlankLine
\BlankLine
\BlankLine
\end{algorithm}
\end{minipage}
\qquad
\begin{minipage}{0.48\textwidth}
\begin{algorithm}[H]
\small
\SetKwInOut{Globals}{Globals}
\SetKwInOut{Locals}{Locals}
\setcounter{algocf}{-1}
\renewcommand{\thealgocf}{}
\SetAlgorithmName{Benchmark}{algorithm}
\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{\emph{opt\_lock}($n$), for $2$ processes and $n$ attempts}
\Globals{
$\mathit{int}~\mathsf{last\_id}, x$\\
}
\BlankLine
\tcp{--------- Process $0< j<2$ ---------}
\Locals{$\mathit{int}~i$}
%\BlankLine
$i\gets 0$\\
\While{$i< n$}{
$i\gets i+1$\\
$\mathsf{last\_id}\gets j$\\
$x\gets \mathsf{get\_message}(j)$\\
\uIf{$\mathsf{last\_id}=j$}{
\Return $x$
}
}
\Return -1
\BlankLine
\BlankLine
\BlankLine
\end{algorithm}
\end{minipage}


==> definitions_bk.tex <==
\section{Preliminaries}\label{sec:prelim}

\newcommand{\es}{\xi}
\newcommand{\eqc}{\sim}
\newcommand{\ihb}[1]{{#1}^{!}}  %imm hb (precedes)
\newcommand{\ihbm}{\ihb{<}} %imm hb m-trace


%TODO: get rid of \prgo
\newcommand{\po}{\leq_{P}}
\newcommand{\espo}{\preceq}
\newcommand{\prgo}{\po}
\newcommand{\exc}{\#}
\newcommand{\obs}{O}
\newcommand{\sca}{\Pi}
\newcommand{\mhbet}{Hbet}
\newcommand{\GlobalV}{\mathsf{G}}
\newcommand{\LocalV}{mathsf{L}}
\newcommand{\Programm}{\mathcal{P}}

\newcommand{\nssays}[1]{{\bf NS:} #1}



\begin{comment}
concurrent system (set of threads, state, enabled events in a state, happens-before events, event structure (glynn winskel), sequential consistency).


event structure (E, exclusivity, hb). 
each event has (loc, val, en)
 abstraction: e and e’ are exclusive if en(e) /\ en(e’) is infeasible. e.g., if they occur in different branches of a condition 


Formalize: observer relation. interference relation?
Formalize: notion of equivalence relations based on O, HB, ..
\end{comment}


%event structures, incompatible event sets to model events on different branches, %how to obtain event structures from programs



A (strict) partial-order relation $<$ over set $S$ is an irreflexive, asymmetric and transitive relation over $S\times S$.
A {\it linearization} of $<$ is a totally ordered relation $<'$ such that for all $s_1, s_2\in S$, $s_1 < s_2 \Rightarrow s_1 <' s_2$.

A binary relation $\eqc$ on a set $X$ is an equivalence relation iff $\eqc$ is reflexive, symmetric and transitive. 
Given $x\in X$, let $[x]$ denote the equivalence class of $x$ under $\eqc$ such that $\forall y\in[x]~.~x\eqc y$.
The {\it quotient set} of $X$ under $\eqc$ is the set of all possible equivalence classes of X under $\eqc$ is $X/\eqc := \{[x]\ |\ x\in X\}$.

{\bf Concurrent Programs.} 
A concurrent program $P$ consists of a set of threads $T_i$ ($i>0$).
Each thread is defined over a set of local variables $L_i$
Threads communicate using a set of shared variables $G$.
The {\it state} of a program $P$ consists of valuation of shared variables $G$ and the local variables $L_i$ of each thread.

We model each thread as a control flow graph over {\tt assume}, {\tt assign} and {\tt assert} statements.
An {\it atomic} block in the CFG consists of set of statements which must execute without any interference.
To simplify, synchronization statements, e.g., {\tt lock/unlock}, {\tt wait/notify} are also modeled using {\tt assume} and {\tt assign}. 
For example, {\tt lock(A)} in thread $T_i$ ($i > 0$) translates to an atomic block \{{\tt assume (A == 0); A = i;}\} and {\tt unlock(A)} in thread $T_i$ translates to ({\tt A := 0}).
%Here, the {\tt assert} statement is only required if we check for erroneous unlocks.
To keep discussion focused on concurrency, we will only consider programs over integer variables.
Details on handling various program constructs, e.g., pointers, and sequential aspects, e.g., function calls, and handling fork/join calls can be found in literature, e.g.,~\cite{SW10}.


{\bf see http://www.cl.cam.ac.uk/~gw104/TraceG2a.pdf}

{\bf Event structure.}
An execution of a concurrent program $P$ gives rise to {\it events} of multiple kinds: a {\it read} or {\it write} to a memory location (memory access events), thread creation ({\it fork}) and termination ({\it join}) events, and so on.
We model the set of executions of a concurrent program $P$ using the notion of an event structure (similar to ~\cite{winskel})
An {\it event structure} $\es = (E, \espo, \exc)$ consists of a set of events $E$, a partial order $\espo$ on $E$, and a binary, irreflexive and symmetric relation $\exc$ called the {\it exclusivity} relation.
We define $[e] = \{e' | e'\espo e\}$ be the {\it downward closure} of $e$ in $E$.



Given the control flow graph (CFG) of a concurrent program $P$, we can obtain its event structure $\es = (E,\espo,\exc)$ via CFG transformations\cite{SW10,danielCAV13}.
The set $E$ is the set of events from $P$, the partial order $\espo$ is the union of the program ordering relation among intra-thread statements as well as inter-thread ordering relation due to fork-join statements and $\exc$ contains events that cannot co-occur in a program execution, e.g., those arising from statements on different branches of a conditional statement.
In the following, to analyze parallel thread interactions, we will consider event structures over {\it global} events only, i.e., reads/writes to shared variables (global reads/writes), fork and join events.



Given a structure $\es = (E,\po,\exc)$ for $P$, a (partial) execution of $P$ is modeled by a configuration $C\subseteq E$ where \\
(i) $\forall e_1, e_2\in E', \neg(\exc(e_1,e_2))$ (contains no exclusive events), \\
(ii) $\forall e\in C$, $[e] \subseteq C$ ($C$ is downward-closed). 
Note that every (partial) program {\it execution trace} $t$ (trace, in short) of $P$ corresponds to a linearization of the events in some configuration $C$ of $\es$.

We additionally define a set of properties for each read/write (memory access) event $e$: $loc(e)$, $val(e)$.
Memory access events $e_1$ and $e_2$ are said to {\it conflict}, denoted by $confl(e_1,e_2)$, iff $loc(e_1) = loc(e_2)$ and either $e_1$ or $e_2$ is a write.
For convenience, we will denote read and write events using letters $r$ and $w$ respectively.
Given a set of events $E$, $E_r, E_w\subseteq E$ denote the read and write event subsets of $E$ respectively.


%Each event $e$ is associated with an enabling predicate $en(e)$




{\bf Sequential consistency~\cite{L79}.} each read must observe the last write to the same memory location. imposes a fixed global ordering between writes to a memory location.
Now the SC axioms ($HB$ also satisfies partial order axioms, DEFINE $Hbet$ using $HB$).


\[\begin{array}{l}
\sca := \exists HB.~~\sca_0\wedge\sca_1 \\
\sca_{0} := \forall e_1, e_2\in E.~~(e_1 \prgo e_2) \Rightarrow HB(e_1,e_2) \\
\sca_1 := \forall r \in E_r~ \exists w\in E_w.~~\phi_1(r,w)\wedge\phi_2(r,w) \\
\phi_1 (r,w) := (loc(r) = loc(w) \wedge val(r) = val (w) \wedge HB(w,r)) \\
\phi_2 (r,w) := \forall w'\in E_w.~\mhbet(w,w',r)\Rightarrow loc(r) \neq loc(w') 
\end{array}\]

Observe that we can rewrite $\sca_1$ using an {\it observer} function $\obs(r): E_r \rightarrow E_w$:
$$\sca'_1 := \exists O.\forall r\in E_r. \phi_1(r, O(r))\wedge \phi_2(r, O(r))$$.
The observer function forms the basis of memory consistency specifications of concurrent systems~\cite{AG96}; intuitively, $O(r) = w$ if read $r$ returns the value written by $w$.

Given a configuration $C$ of an event structure $\es=(E,\espo,\exc)$, we say that $C$ is {\it sequentially consistent} iff $\sca$ is satisfiable with $HB = \espo$ and we can find a witness $O$ so that $O(r) = w$ ($w \in C$) for each $r\in C$.

We define a {\it data trace} $d = (C,O)$ as a tuple over a configuration $C$ and observer function $O$.
A data trace $d$ is said to be SC iff $\espo$ and $O$ satisfy $\sca$, 

\nssays{Confused here. Is $O$ uniquely defined by a sequentially consistent $C$?? Do $O$ and $E$ imply we can compute an unique $\espo$? If yes, then we can get SC traces simply using $O$, no HB required.}


{\bf Mazurkiewicz-traces.}
The formalism of Mazurkiewicz(M)-traces~\cite{M86} views a distributed system as a set of concurrently executing events, some of which may be dependent.
Formally, a Mazurkiewicz trace $M$ is a tuple $(E,<, D)$, where $E$ is a set of events, $<$ is a strict partial order over $E$ and $D\subseteq E\times E$ is a reflexive and symmetric {\it dependence} relation.
Let $\ihbm$ be the {\it immediate precedence relation}.% (intuitively, the minimal partial order).
We say that $e$ immediately precedes $e'$, denoted  $e\ihbm e'$, iff $e < e'$ and there is no $x$ with $e < x < e'$.

M-traces have been widely used in enumerative analysis of concurrent systems.
However, they do not distinguish between read or write events directly, but instead model read-write interactions using dependence relation $D$.

%{\it M-traces use dependency between co-occuring events while configurations use $O$}




==> enumerative_bk.tex <==
\section{Data-centric Dynamic Partial Order Reduction}\label{sec:enumerative}

In this section we develop our data-centric DPOR algorithm called $\EnumExplore$ and prove its correctness and compactness,
namely that that the algorithm explores exactly one maximal trace from each equivalence class of the quotient of the trace space modulo the observation equivalence $\TraceSpace/\sim_{\Obs}$.






\subsection{Data-centric Dynamic Partial Order Reduction}\label{subsec:dcdpor}

\smallskip\noindent{\bf Algorithm $\EnumExplore$.}
We are now in position to describe our data-centric DPOR algorithm.
The algorithm receives as input a maximal trace $\Trace$ and annotation pair $\Annotation=(\Annotationpos, \Annotationneg)$,
such that $\Trace$ is compatible with $\Annotationpos$.
The algorithm scans $\Trace$ to detect conflicting read-write pairs of events that are not annotated, i.e, a read even $\Read\in \Reads{\Trace}$ and a write event $\Write\in\Writes{\Trace}$ such that $\Read\not\in\Domain(\Annotationpos)$ and $\ConflRW(\Read, \Write)$.
If $\Write\not \in \Annotationneg(\Read)$, then $\EnumExplore$ will try to \emph{mutate} $\Read$ to $\Write$, i.e., the algorithm will push $(\Read, \Write)$ in the positive annotation $\Annotationpos$ and call $\Realize$ to obtain a trace that realizes the new positive annotation.
call itself recursively with the new annotation as input.
If the recursive call succeeds, then the algorithm will push $\Write$ to the negative annotations of $\Read$,
i.e., will insert $\Write$ to $\Annotationneg(\Read)$.
This will prevent further recursive calls from pushing $(\Read, \Write)$ into their positive annotations.
\cref{algo:enumerative} provides a formal description of $\EnumExplore$.
Initially, $\EnumExplore$ is executed on input $(\Trace,\Annotation)$ where $\Trace$ is an arbitrary maximal trace of $\System$,
and $\Annotation=(\emptyset,\emptyset)$ is a pair of empty annotations.

%\begin{algorithm}%[H]
%\small
%%\SetAlgoNoLine
%\DontPrintSemicolon
%%\setstretch{1.05}
%\caption{$\EnumExplore(\Trace, \Annotation)$}\label{algo:enumerative}
%\KwIn{A maximal trace $\Trace$, an annotation pair $\Annotation=(\Annotationpos, \Annotationneg)$}
%\BlankLine
%\tcp{Iterate over reads not yet mutated}
%\ForEach{$\Read\in \Events{\Trace}\setminus \Domain(\Annotationpos)$ in increasing index $\Index_{\Trace}(\Read)$}{\label{line:foreachread}
%\tcp{Find conflicting writes allowed by $\Annotationneg$}
%\ForEach{$\Write\in \Events{\Trace}$ s.t. $\Confl(\Read, \Write)$ and $\Write\not \in \Annotationneg(\Read)$}{\label{line:foreachwrite}
%$\Annotationpos_{\Read, \Write}\gets \Annotationpos\cup \{(\Read, \Write)\}$ \label{line:strengthenpos} \\
%\tcp{Attempt mutation and update $\Annotationneg$}
%Let $\Trace'\gets \Realize(\Annotationpos_{\Read, \Write})$\label{line:get_trace}\\
%\uIf{$\Trace'\neq \bot $}{
%$\Trace''\gets$ a maximal extension of $\Trace'$\\
%$\Annotationneg(\Read)\gets \Annotationneg(\Read)\cup \{\Write\}$\label{line:strengthenneg}\\
%$\Annotation_{\Read, \Write}\gets (\Annotationpos_{\Read, \Write}, \Annotationneg)$\\
%Call $\EnumExplore(\Trace'', \Annotation_{\Read,\Write})$ 
%}
%}
%}
%\end{algorithm}


\begin{algorithm}%[H]
\small
%\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\EnumExplore(\Trace, \Annotation)$}\label{algo:enumerative}
\KwIn{A maximal trace $\Trace$, an annotation pair $\Annotation=(\Annotationpos, \Annotationneg)$}
\BlankLine
\tcp{Iterate over reads not yet mutated}
\ForEach{$\Read\in \Events{\Trace}\setminus \Domain(\Annotationpos)$ in increasing index $\Index_{\Trace}(\Read)$}{\label{line:foreachread}
\tcp{Find conflicting writes allowed by $\Annotationneg$}
\ForEach{$\Write\in \Events{\Trace}$ s.t. $\ConflRW(\Read, \Write)$ and $\Write\not \in \Annotationneg(\Read)$ and $\Obs_{\Trace}(\Read)\neq \Write$}{\label{line:foreachwrite}
$\Annotationpos_{\Read, \Write}\gets \Annotationpos\cup \{(\Read, \Write)\} \cup\{(\Read',\Obs_{\Trace}(\Read')):~\Read'\in \Past_{\Trace}(\Read)\cup \Past_{\Trace}(\Write)\}$ \label{line:strengthenpos} \\
\tcp{Attempt mutation and update $\Annotationneg$}
Let $\Trace'\gets \Realize(\Annotationpos_{\Read, \Write})$\label{line:get_trace}\\
\uIf{$\Trace'\neq \bot $}{
$\Trace''\gets$ a maximal extension of $\Trace'$\\
$\Annotationneg(\Read)\gets \Annotationneg(\Read)\cup \{\Write\}$\label{line:strengthenneg}\\
$\Annotation_{\Read, \Write}\gets (\Annotationpos_{\Read, \Write}, \Annotationneg)$\\
Call $\EnumExplore(\Trace'', \Annotation_{\Read,\Write})$ 
}
}
}
\end{algorithm}



We say that $\EnumExplore$ \emph{explores} a class of $\TraceSpace/\sim_{\Obs}$ when it is called on some annotation input $\Annotation=(\Annotationpos, \Annotationneg)$, where $\Annotationpos$ is realized by some (and hence, every) trace in that class.
The following two lemmas show the optimality of $\EnumExplore$, namely that the algorithm explores every such class at most once (\emph{compactness}) and at least once (\emph{completeness}).

\smallskip
\begin{lemma}[Compactness]\label{lem:compactness}
Consider any two executions of $\EnumExplore$ on inputs $(\Trace_1, \Annotation_1)$ and $(\Trace_1,\Annotation_2)$.
Then $\Annotationpos_1\neq \Annotationpos_2$.
\end{lemma}
\begin{proof}
Examine the recursion tree $\RecTree$ generated by $\EnumExplore$, where every node $u_i$ is labeled with the trace $\Trace_{i}$ and annotation input $\Annotation_i=(\Annotationpos_i, \Annotationneg_i)$ given to $\EnumExplore$.
If $u_1$ is an ancestor of $u_2$, then when $\EnumExplore$ was executed on input $(\Trace_1,\Annotation_1)$,
a read $\Read\not\in \Domain(\Annotationpos_1)$ created $\Annotationpos_{\Read,\Write}$ in \cref{line:strengthenpos} on the branch from $u_1$ to the direction of $u_2$ in $\RecTree$. Since the algorithm never removes pairs $(\Read, \Write)$ from the positive annotations,
we have that $\Read\in \Domain(\Annotationpos_2)$.
A similar analysis holds if $u_2$ is an ancestor of $u_1$.
Now consider the case that $u_1$ and $u_2$ do not have an ancestor relationship.
Let $u_j$ be the lowest common ancestor of $u_1$ and $u_2$ in $\RecTree$,
and $u_{j_1}$ (resp. $u_{j_2}$) the child of $u_j$ in the direction of $u_1$ (resp. $u_2$).
Let $\Read_1$ (resp. $\Read_2$) be the read on \cref{line:strengthenpos} that generated
$\Annotationpos_{j_1}$ (resp. $\Annotationpos_{j_2}$), i.e.,
\[
\Annotationpos_{j_1}=\Annotationpos_{j}\cup \{(\Read_1, \Write_1)\} \quad \text{and} \quad \Annotationpos_{j_2}=\Annotationpos_{j}\cup \{(\Read_2, \Write_2)\}
\]
If $\Read_1=\Read_2$ then $\Write_1\neq \Write_2$, thus $\Annotationpos_{j_1}(\Read)\neq \Annotationpos_{j_2}$,
and since the algorithm never removes pairs $(\Read,\Write)$ from positive annotations we have that
$\Annotationpos_1(\Read)\neq \Annotationpos_2(\Read)$.
Now assume that $\Read_1\neq \Read_2$.
If $u_{j_1}=u_1$, then $\Read_2\not \in \Domain(\Annotationpos_1)$, whereas $\Read_2\in \Domain(\Annotationpos_2)$.
Similarly if $u_{j_2}=u_2$.
Finally, if $u_{j_1}\neq u_1$ and $u_{j_2}\neq u_2$, 
assume w.l.o.g. that $\Index_{\Trace_j}(\Read_1)< \Index_{\Trace_j}(\Read_2)$.
%where $\Trace'$ is the trace returned by $\Realize$ in \cref{line:get_trace} when $\EnumExplore(\Annotation_{j})$ was executed.
Then, before $\EnumExplore(\Annotation_{j_2})$ is executed, \cref{line:strengthenneg} adds $\Write_1\in \Annotationneg(\Read_1)$,
thus by the condition of \cref{line:foreachwrite}, we have that $(\Read_1, \Write_1)\not\in \Annotationpos_{j'}$,
in all descendants $u_{j'}$ of $u_{j_2}$, and hence $(\Read_1, \Write_1)\not\in \Annotationpos_{2}$.
In all cases we have $\Annotationpos_1\neq\Annotationpos_2$, as desired.
\end{proof}


We now turn our attention to completeness, namely that every realizable observation function is realized by a trace explored by $\EnumExplore$.
The proof assumes that every maximal trace generated by the algorithm is lock-free.
This is a reasonable assumption, as non-lock-free traces are typically considered buggy,
and thus witness erroneous behavior of the system.

\smallskip
\begin{lemma}[Completeness]\label{lem:completeness}
For every realizable observation function $\Obs$, $\EnumExplore$ generates a trace $\Trace$ that realizes $\Obs$.
\end{lemma}
\begin{proof}
Let $\RecTree$ be the recursion tree of $\EnumExplore$.
Given a node $u$ of $\RecTree$, we denote by $\Trace_u$ and $\Annotation_u=(\Annotationpos_u, \Annotationneg_u)$ the input of $\EnumExplore$ on $u$. Recall that $\Trace_u$ is compatible with $\Annotationpos_u$, thus it suffices to show
that $\EnumExplore$ is called with a positive annotation being equal to $\Obs$.
We define a traversal on $\RecTree$ with the following properties:
\begin{compactenum}
\item\label{item:agreement} If $u$ is the current node of the traversal, then $\Annotationpos_u\subseteq \Obs$.
\item\label{item:progress} If  $\Annotationpos_u\subset \Obs$, then the traversal proceeds either
\begin{compactenum}
\item\label{item:child} to a node $v$ of $\RecTree$ with $\Annotationpos_u\subset \Annotation_v$,
\item\label{item:other} to some other node of $\RecTree$,
\end{compactenum}
and \cref{item:other} happens a finite number of times.
\end{compactenum}
Observe that every time the traversal executes \cref{item:child}, $\Obs$ agrees with
$\Annotationpos_v$ on more reads than $\Annotationpos_u$ (in particular, one more read).
Since \cref{item:other} is executed a finite number of times, any such traversal is guaranteed to reach a node $w$ with $\Annotation_w=\Obs$. 

The traversal starts from $u$ being the root of $\RecTree$,
and \cref{item:agreement} holds as then $\Annotationpos_u=\emptyset\subseteq \Obs$.
Now consider that the traversal is on any node $u$ that satisfies \cref{item:agreement}.
and recall that trace $\Trace_u$ is a maximal trace that realizes $\Annotationpos_u$.
Let $\Trace^{*}$ be a trace that realizes $\Obs$, and $\Read$ be the first read of $\Trace^{*}$ not in $\Annotationpos_u$, i.e.,
\[
\Read=\arg\min_{\Read'\in \Events{\Trace^{*}}\setminus\Domain(\Annotationpos_u)} \Index_{\Trace^{*}}(\Read')
\]
and $\Write=\Obs_{\Trace^{*}}(\Read)$.
Then for every $\Read'\in \Past_{\Trace^{*}}(\Read)$, we have $\Index_{\Trace^{*}}(\Read')<\Index_{\Trace^{*}}(\Read')$
and thus $\Read'\in \Events{\Trace_u}$ and $\Obs_{\Trace^{*}}(\Read')=\Obs_{\Trace_u}(\Read')$.
By \cref{lem:obs_to_enable_max}, we have $\Read\in \Events{\Trace}$.
Since $\Index_{\Trace^{*}}(\Write)<\Index_{\Trace^{*}}(\Read)$, a similar argument yields that $\Write\in \Events{\Trace}$.
We now distinguish two cases, based on whether $\Write\in \Annotationneg_u(\Read)$ or not.
\begin{compactenum}
\item If $\Write\not \in \Annotationneg_u(\Read)$, then in \cref{line:get_trace} the algorithm will generate a trace $\Trace'$ that is compatible with the strengthened annotation $\Annotationpos_u\cup(\Read, \Write)$, and call itself recursively on some child $v$ of $u$
with $\Annotationpos_v=\Annotationpos_u\cup(\Read, \Write)$.
The traversal proceeds to $v$ and \cref{item:agreement} holds, as desired.

\item If $\Write\in \Annotationneg_u(\Read)$, 
then there exists a highest ancestor $x$ of $u$ in $\RecTree$ where $\EnumExplore$ was called with
$(\Read, \Write)\in \Annotationneg_x$.
Following \cref{line:strengthenneg}, this can only have happened if 
$x$ has a sibling $v$ in $\RecTree$ with $(\Read, \Write)\in \Annotationpos_v$.
Let $z$ be the parent of $x,v$, and we have $\Annotationpos_z\subset \Annotationpos_u\subset \Obs$,
and $\Annotationpos_v=\Annotationpos_z \cup (\Read,\Write)\subseteq \Obs$.
Thus, the traversal proceeds to $v$ and \cref{item:agreement} holds, as desired.
In this case, we say that the traversal \emph{backtracks to $x$ through $z$}.
\end{compactenum}

Finally, we argue that \cref{item:other} will only occur a finite number of times in the traversal.
Since $\RecTree$ is finite, it suffices to argue that the traversal backtracks through any node $z$ a finite number of times.
Indeed, fix such a node $z$ and let $x_1,x_2,\dots$ be the sequence of (not necessarily distinct) children of $z$ that the traversal backtracks to, through $z$.
Let $\Read_i$ be the unique read in $\Domain(\Annotationpos_{x_i})\setminus\Domain(\Annotationpos_{z})$.
By \cref{line:foreachread}, we have that $\Index_{\Trace_z}(\Read_{i+1}) < \Index_{\Trace_z}(\Read_i)$, hence no node repeats in the sequence $(x_i)_i$,
and thus the traversal backtracks through $z$ a finite number of times.
The desired result follows.
\end{proof}


\smallskip
\begin{theorem}\label{them:enum_explore}
Consider a concurrent system $\System$ of $k$ processes on an acyclic space,
and $n=\max_{\Trace\in\TraceSpace}|\Trace|$ the maximum length of a trace.
The algorithm $\EnumExplore$ explores each class of $\TraceSpace/\sim_{\Obs}$ exactly once,
and requires $O\left(|\TraceSpace/\sim_{\Obs}|\cdot n \cdot k\right)$ time.
\end{theorem}
\begin{proof}
\cref{lem:compactness} and \cref{lem:completeness} guarantee the optimality of $\EnumExplore$, 
i.e., that $\EnumExplore$ explores each class of $\TraceSpace/\sim_{\Obs}$ exactly once.
The time spent in exploring each class is the time required to generate a trace $\Trace'$ that realizes the positive annotation in
\cref{line:get_trace}. By \cref{lem:trace_feasibility}, this requires linear time in the number of conflicting pairs in $\Trace'$,
which is bounded by $n\cdot k$.
The desired result follows.
\end{proof}


==> enumerative_efficient.tex <==
\section{Efficient Data-centric Dynamic Partial Order Reduction}\label{sec:enumerative_efficient}

In the current section we introduce some modifications to our $\EnumExplore$ algorithm that greatly improve the efficiency of the exploration of the trace space.


\smallskip\noindent{\bf Annotated causal cones.}
Given an annotation $\Annotationpos$, a trace $\Trace$ compatible with $\Annotationpos$, and some event $\Event\in \Events{\Trace}$, the \emph{annotated causal past cone} $\APast_{\Trace}(\Event)$ of $\Event$ in $\Trace$ is a a set that contains the following events (and only those):
\begin{compactenum}
\item if there is an event $\Event'\in\Events{\Trace}$ with $\PS(\Event',\Event)$, then $\Event'\in \APast_{\Trace}(\Event)$,
\item if $\Event_1\in \APast_{\Trace}(\Event)$, for every event $\Event_2\in \Events{\Trace}$ such that
$\PS(\Event_2, \Event_1)$, we have that $\Event_2\in \APast_{\Trace}(\Event)$, and
\item if there exists a read $\Read\in \APast_{\Trace}(\Event)\cap \SysReads$,
we have that $\Annotationpos(\Read)\in \APast_{\Trace}(\Event)$.
\end{compactenum}
Note that the definition of the annotated causal past cone of $\Event$ in $\Trace$ is similar to that of the causal past cone of $\Event$ in $\Trace$, where the observation in Item~3 $\Obs_{\Trace}(\Read)$ has been replaced by the annotation $\Annotationpos(\Read)$.
The \emph{annotated causal future cone} of $\Event$ in $\Trace$ is defined as
\[
\AFuture_{\Trace}=\{\Event'\in \Events{\Trace}:~\Event\in \APast_{\Trace}(\Event')\}
\]


\smallskip\noindent{\bf Conditional negative annotation.}
A \emph{conditional negative annotation} is a partial function $\CondAnnotationneg: \SysReads\times \SysWrites \pto 2^{\SysReads}$
such that if $\CondAnnotationneg(\Read,\Write)=\{\Read_i\}_i$, then $\Location(\Read)=\Location(\Write)=\Location(\Read_i)$ for all $i$.
Conditional negative annotations are used by our efficient algorithm in a similar way that the negative annotations of \cref{sec:enumerative} are used, namely to avoid repeating the same mutations in different branches of the recursive search.
Intuitively, setting $\CondAnnotationneg(\Read,\Write)=\{\Read_i\}_i$ has the effect that the algorithm will not attempt to mutate $\Read\to \Write$, unless $\CondAnnotationneg(\Read,\Write)\cap \Domain(\Annotationpos)\neq \emptyset$, i.e., some $\Read_i$ has been mutated already.


\input{fig_mutations}

\smallskip
\begin{algorithm}%[H]
\small
%\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\EnumExploreEff(\Trace, \Annotation)$}\label{algo:enumerative2}
\KwIn{A pair of trace and annotation $(\Trace, \Annotation=(\Annotationpos, \Annotationneg))$}
\BlankLine
\While{$\exists \Event\in \Enabled(\Trace)$}{\label{line:while_extend}
Extend $\Trace$ by $\Event$\\
\uIf{$\Event$ is a write $\Write$}{\label{line:extend_write}
\tcp{1. Consider all mutations by $\Write$}
\ForEach{$\Read\in \Events{\Trace}\setminus\Domain(\Annotationpos)$ with $\ConflRW(\Read, \Write)$ and $\Obs_{\Trace}(\Read)\neq \Write$ and $\Annotationneg(\Read,\Write)\cap \Domain(\Annotationpos)\neq \emptyset$}{
$\SysReads_{(\Read, \Write)}\gets \{(\Read',\Obs_{\Trace}(\Read')):~\Read'\in \Past_{\Trace}(\Read)\setminus(\Domain(\Annotationpos))\cup \Past_{\Trace}(\Write)\}$\\
%$\Annotationpos_{\Read, \Write}=\Annotationpos \cup\{(\Read, \Write)\} \cup \{(\Read_i, \Obs_{\Trace}(\Read_i)):~\Read_i\in \Past_{\Trace}(\Read)\cup \Past_{\Trace}(\Write) \}$\\
$\Annotationpos_{\Read, \Write}\gets \Annotationpos\cup \{(\Read, \Write)\} \cup \SysReads_{\Read, \Write}$ \label{line:strengthenpos_past} \\
$\Trace'\gets \MutatePost(\Trace, \Read, \Write, \Annotationpos_{\Read, \Write})$\label{line:mutate_post}\\
\uIf{$\Trace' \neq \eps$}{
$\Annotationpos_{\Read,\Write}\gets \Annotationpos_{\Read,\Write} \cup \{(\Read, \Write)\}$\\
$\Annotationneg(\Read, \Write)\gets \Annotationneg(\Read)\cup \SysReads_{\Read, \Write}$\\
Call $\EnumExplore(\Trace', (\Annotationpos_{\Read, \Write}, \Annotationneg))\label{line:push_mutate_post}$
}
}
}
\uIf{$\Event$ is a read $\Read$}{\label{line:extend_read}
\tcp{2. Push $\Obs_{\Trace}(\Read)$ in $\Annotationpos$}
$\Annotationpos_{\Read}\gets \Annotationpos \cup \{(\Read', \Obs_{\Trace}(\Read'):~\Read'\in\OPast_{\Trace}(\Read)\}$\\
$\Annotationneg(\Read)\gets \Annotationneg(\Read)\cup\{\Write\}$\\
Call $\EnumExplore(\Trace, (\Annotationpos_{\Read}, \Annotationneg))$\label{line:push_obs}\\
\tcp{3. Consider all mutations on $\Read$}
\ForEach{$\Write\in \Events{\Trace}\setminus\Annotationneg(\Read)$ with $\ConflRW(\Read, \Write)$}{
Let $\Annotationpos_{\Read, \Write}=\Annotationpos \cup \{(\Read', \Obs_{\Trace}(\Read')):~\Read_i\in \Past_{\Trace}(\Read)\cup \Past_{\Trace}(\Write) \}$\\
$\Trace'\gets \MutatePre(\Trace, \Read, \Write, \Annotationpos_{\Read, \Write})$\label{line:mutate_pre}\\
\uIf{$\Trace' \neq \eps$}{
$\Annotationpos_{\Read,\Write}\gets \Annotationpos_{\Read,\Write} \cup \{(\Read, \Write)\}$\\
$\Annotationneg(\Read)\gets \Annotationneg(\Read)\cup\{\Write\}$\\
Call $\EnumExplore(\Trace', (\Annotationpos_{\Read, \Write}, \Annotationneg))\label{line:push_mutate_pre}$
}
}
}
}
\end{algorithm}



\smallskip
\begin{algorithm}%[H]
\small
%\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\MutatePost(\Trace, \Read, \Write, \Annotationpos)$}\label{algo:mutatepost}
\KwIn{A trace $\Trace$, a read and write $\Read, \Write\in \Events{\Trace}$ with $\HB{\Read}{\Trace}{\Write}$, a positive annotation $\Annotationpos$}
\KwOut{A trace $\Trace'$ with $\Read,\Write \in \Events{\Trace'}$ and $\Obs_{\Trace'}(\Read)=\Write$ or $\eps$}
\BlankLine
\eIf{$\Read\in \Past_{\Trace}(\Write)$ or $\OFuture_{\Trace}(\Read)\cap \Domain(\Annotationpos)\neq \emptyset$}{\label{line:post_if}
\Return $\eps$
}{
Let $\Trace'\gets \Trace\Project \Events{\Trace}\setminus \OFuture_{\Trace}(\Read)$\label{line:post_minus_future}\\
Extend $\Trace'$ with $\Read$\label{line:post_extend}\\
\Return $\Trace'$
}
\end{algorithm}




\smallskip
\begin{algorithm}%[H]
\small
%\SetAlgoNoLine
\DontPrintSemicolon
%\setstretch{1.05}
\caption{$\MutatePre(\Trace, \Read, \Write, \Annotationpos)$}\label{algo:mutatepre}
\KwIn{A trace $\Trace$, a read and write $\Read, \Write\in \Events{\Trace}$ with $\HB{\Write}{\Trace}{\Read}$ and $\Obs_{\Trace}(\Read)\neq \Write$, a positive annotation $\Annotationpos$}
\KwOut{A trace $\Trace'$ with $\Read,\Write \in \Events{\Trace'}$ and $\Obs_{\Trace'}(\Read)=\Write$ or $\eps$}
\BlankLine
Let $W\gets \{\Write_i\in \Trace:~ \Confl(\Write_i, \Read) \text{ and } \Index_{\Trace}(\Write)<\Index_{\Trace}(\Write_i)< \Index_{\Trace}(\Read)$\\
Let $P\gets  \Past_{\Trace}(\Read) \cup \bigcup_{\Read_i\in \Domain(\Annotationpos)}\OPast_{\Trace}(\Read_i)$\\
\eIf{$W\cap P\cap \Future_{\Trace}(\Write)\neq \emptyset$}{
\Return $\eps$
}{
Let $\Trace'\gets \Trace$\\
\While{$\exists \Write_i\in W\setminus P$}{
Let $W\gets W\setminus\{\Write_i\}$\\
Let $\Trace'\gets \Trace\Project \Events{\Trace'}\setminus \OFuture_{\Trace'}(\Write_i)$
}
Let $\Annotationpos_{\Read,\Write}\gets \Obs_{\Trace'}\cup \{(\Read,\Write)\}$\\
Let $\Trace''\gets \Realize(\Annotationpos_{\Read,\Write})$\\
\lIf{$\Trace''\neq \bot$}{
\Return $\Trace''$
}
\Return $\eps$\\
}
\end{algorithm}



\begin{lemma}\label{lem:compactness2}
Consider any two executions of $\EnumExploreEff$ on inputs $\Annotation_1=(\Annotationpos_1, \Annotationneg_1)$ and $\Annotation_2=(\Annotationpos_2, \Annotationneg_2)$.
Then $\Annotationpos_1\neq \Annotationpos_2$.
\end{lemma}
\begin{proof}
The proof is similar to that of \cref{lem:compactness}.
\end{proof}


\begin{lemma}\label{lem:completeness2}
For every realizable observation function $\Obs$, $\EnumExploreEff$ generates a trace $\Trace$ such that
$\Obs_{\Trace}=\Obs$.
\end{lemma}
\begin{proof}
The proof is similar to that of \cref{lem:completeness}. 
Let $\RecTree$ be the recursion tree of $\EnumExploreEff$.
Given a node $u$ of $\RecTree$, we denote by $(\Trace_u, \Annotation_u=(\Annotationpos_u, \Annotationneg_u))$ the input of $\EnumExploreEff$ on $u$.
It is easy to verify that $\Annotationpos_u\subseteq \Obs_{\Trace_u}$ for every node $u$.
We again define a traversal on $\RecTree$ with the following properties:
\begin{compactenum}
\item\label{item:agreement2} If $u$ is the current node of the traversal, then $\Annotationpos_u\subseteq \Obs$.
\item\label{item:progress2} If  $\Annotationpos_u\subset \Obs$, then the traversal proceeds either
\begin{compactenum}
\item\label{item:child2} to a node $v$ of $\RecTree$ with $\Annotationpos_u\subset \Annotation_v$,
\item\label{item:other2} to some other node of $\RecTree$,
\end{compactenum}
and \cref{item:other2} happens a finite number of times.
\end{compactenum}

The traversal starts from $u$ being the root of $\RecTree$,
and \cref{item:agreement} holds as then $\Annotationpos_u=\emptyset\subseteq \Obs$ and $\Trace_u=\eps$.
Now consider that the traversal is on a node $u$ that satisfies \cref{item:agreement2}.
\cref{line:while_extend} extends $\Trace_u$ to a maximal trace $\Trace$, and since $\Annotationpos_u\subseteq \Obs_{\Trace_u}$,
we have $\Annotationpos_u\subseteq \Obs_{\Trace}$.
Let $\Trace^{*}$ be a trace that realizes $\Obs$, and $\Read$ be the first read of $\Trace^{*}$ not in $\Annotationpos_u$, i.e.,
\[
\Read=\arg\min_{\Read'\in \Events{\Trace^{*}}\setminus\Domain(\Annotationpos_u)} \Index_{\Trace^{*}}(\Read')
\]
and $\Write=\Obs_{\Trace^{*}}(\Read)$.
Then for every $\Read'\in \Past_{\Trace^{*}}(\Read)$, we have $\Index_{\Trace^{*}}(\Read')<\Index_{\Trace^{*}}(\Read')$
and thus $\Read'\in \Events{\Trace_u}$ and $\Obs_{\Trace^{*}}(\Read')=\Obs_{\Trace}(\Read')$.
By \cref{lem:obs_to_enable_max}, we have $\Read\in \Events{\Trace}$.
Since $\Index_{\Trace^{*}}(\Write)<\Index_{\Trace^{*}}(\Read)$, a similar argument yields that $\Write\in \Events{\Trace}$.

It is easy to see that if $\Read,\Write\in \Events{\Trace_u}$, then $u$ has a sibling node $v$ in $\RecTree$ such that
$\Annotationpos_v=\Annotationpos_u\cup \{(\Read,\Write)\}$.
For the remaining of the proof we assume that 
$\Read\in\Events{\Trace}\setminus\Events{\Trace_u}$ or $\Write\in\Events{\Trace}\setminus\Events{\Trace_u}$ (or both).
Thus, $\EnumExploreEff$ will detect a potential mutation on $\Read$ by $\Write$ in either \cref{line:extend_read} or \cref{line:extend_write},
depending on whether $\HB{\Write}{\Trace}{\Read}$ or $\HB{\Read}{\Trace}{\Write}$.
We now distinguish two cases, based on whether $\Write\in \Annotationneg_u(\Read)$ or not.

\begin{compactenum}
\item If $\Write\not\in \Annotationneg_u(\Read)$, we distinguish two cases, based on whether $\HB{\Read}{\Trace}{\Write}$ or not.
\begin{compactenum}
\item If $\HB{\Read}{\Trace}{\Write}$, let $\Trace$ be the extension of $\Trace_u$ with $\Write$ being the last event.
Then we have $\ConflRW(\Read, \Write)$, and $\EnumExploreEff$ calls $\MutatePost(\Trace,\Read,\Write,\Annotationpos_u)$.
Let $\ell=\Index_{\Trace^{*}}(\Read)-1$, and by the induction hypothesis, for every read $\Read'\in\Events{\Trace^{*}[\ell]}$ we have that $\Read'\in \Domain(\Annotationpos_u)$ and $\Obs_{\Trace^{*}}(\Read')=\Annotationpos_u(\Read')=\Obs_{\Trace}(\Read')$.
By \cref{lem:cones} we have $\OPast_{\Trace^{*}[\ell]}(\Read')=\OPast_{\Trace}(\Read')$, and since $\Index_{\Trace^{*}}(\Read')<\Index_{\Trace^{*}}(\Read)$, we have $\Read\not \in\OPast_{\Trace^{*}[\ell]}(\Read')$ and thus $\Read'\not \in \OFuture_{\Trace}(\Read)$. Since for every such $\Read'$ we have $\Read'\in \Domain(\Annotationpos_u)$, we conclude that 
(i)~$\OFuture_{\Trace}(\Read)\cap \Domain(\Annotationpos)= \emptyset$.
Similarly, we have $\OPast_{\Trace^{*}[\ell]}(\Write)=\OPast_{\Trace}(\Write)$ and thus $\Read\not\in \OPast_{\Trace}(\Write)$, which yields that (ii)~$\Read\not\in \Past_{\Trace}(\Write)$.
Statements (i)~and(ii)~guarantee that the condition of \cref{line:post_if} of $\MutatePost$ does not hold, hence $\MutatePost$ does not return $\eps$.
By \cref{lem:cone_ofuture_trace}, $\Trace'$ in \cref{line:post_minus_future} is a trace, and \cref{lem:obs_to_enable_max} guarantees that $\Read\in \Enabled(\Trace')$.
Hence $\MutatePost$ successfully mutates $\Read$ to $\Write$, and the traversal proceeds to the child $v$ of $u$ in $\RecTree$ that corresponds to the recursive call of $\EnumExploreEff$ in \cref{line:push_mutate_post}, after $\MutatePost$ has returned $\Trace'\neq \eps$.
\item If $\HB{\Write}{\Trace}{\Read}$, let $\Trace$ be the extension of $\Trace_u$ with $\Read$ being the last event.
We distinguish two cases, based on whether $\Obs_{\Trace}(\Read)=\Write$ or not. 
In the first case, let $v$ be the node of $\EnumExploreEff$ that corresponds to the recursive call
in \cref{line:push_obs} with $\Annotationpos_v=\Annotationpos_u\cup \{(\Read, \Write)\}$, and let the traversal proceed with node $v$.
Otherwise, we have $\ConflRW(\Read, \Write)$, and $\EnumExploreEff$ calls $\MutatePre(\Trace,\Read,\Write,\Annotationpos_u)$.
Let $\ell=\Index_{\Trace^{*}}(\Read)-1$, and similarly as in Item~1, for every read $\Read'\in\Events{\Trace^{*}[\ell]}$,
we have $\OPast_{\Trace^{*}[\ell]}(\Read')=\OPast_{\Trace}(\Read')$.

{\bf AP: Finish proof}
\end{compactenum}
\item If $\Write\in \Annotationneg_u(\Read)$, the case is similar to the corresponding one in \cref{lem:completeness}.
That is, then there exists a highest ancestor $x$ of $u$ in $\RecTree$ where $\EnumExploreEff$ was called with
$(\Read, \Write)\in \Annotationneg_x$.
This can only have happened if 
$x$ has a sibling $v$ in $\RecTree$ with $(\Read, \Write)\in \Annotationpos_v$.
Let $z$ be the parent of $x,v$, and we have $\Annotationpos_z\subset \Annotationpos_u\subset \Obs$,
and $\Annotationpos_v=\Annotationpos_z \cup (\Read,\Write)\subseteq \Obs$.
Thus, the traversal proceeds to $v$ and \cref{item:agreement2} holds, as desired.
\end{compactenum}

\end{proof}


\smallskip
\begin{theorem}\label{them:enum_explore2}
Consider a concurrent system $\System$ of $k$ processes on an acyclic state space,
and $n=\max_{\Trace\in\TraceSpace}|\Trace|$ the maximum length of a trace of $\System$.
The algorithm $\EnumExplore2$ explores each class of $\TraceSpace/\sim_{\Obs}$ exactly once,
and requires $O\left(|\TraceSpace/\sim_{\Obs}|\cdot n \cdot k\right)$ time.
\end{theorem}


==> experiments_bk.tex <==
\section{Experiments}\label{sec:experiments}

Here we report on the implementation and experimental evaluation of our data-centric DPOR algorithm. 

\subsection{Implementation Details}\label{subsec:implementation}

\smallskip\noindent{\bf Implementation.}
We have implemented our data-centric DPOR in C++,
by extending the tool Nidhugg\footnote{\url{https://github.com/nidhugg/nidhugg}}.
Nidhugg is a powerful tool that utilizes the LLVM compiler infrastructure, 
and hence our treatment of programs is in the level of LLVM's intermediate representation (IR).
Concurrent architectures are supported via POSIX threads.


\smallskip\noindent{\bf Handling static arrays.}
The challenge in handling arrays (and other data structures) lies in the difficulty of determining whether two global events access the same location of the array (and thus are in conflict) or not.
Indeed, this is not evident from the CFG of each process, but depends on the values of indexing variables (e.g. the value of local variable $i$ in an access to $\mathsf{table}[i]$).
DPOR methods offer increased precision, as during the exploration of the trace space, backtracking points are computed dynamically, given a trace, where the value of indexing variables is known.
In our case, the value of indexing variables is also needed when procedure $\Realize$ is invoked to construct a trace which realizes a positive annotation $\Annotationpos$. 
Observe that the values of all such variables are determined by the value function $\Value_{\Annotationpos}$, and thus in every sequential trace $\SeqTrace_i$ of the basis $(\SeqTrace_i)_i$ of $\Annotationpos$ these values are also known.
Hence, arrays are handled naturally by the dynamic flavor of the exploration.

\smallskip\noindent{\bf Handling cyclic architectures.}
In order to effectively handle cyclic architectures, we followed the following process.
Wlog, we considered that the input architecture always has the most difficult topology, namely it is a clique.
First, the cyclic architecture is converted to a star architecture, by choosing some distinguished process $\Process_1$ as the root of the star,
and the remaining processes $\Process_2,\dots \Process_k$ are the leaves.
Recall that a a positive annotation yields a sequential trace for each process.
We use the Mazurkiewicz equivalence to generate all possible Mazurkiewicz-based interleavings between traces of the leaf processes,
and our observation equivalence to generate all possible observation-based interleavings between the root and every leaf process.
Hence the observation equivalence is wrt the star sub-architecture, which is acyclic, and thus our techniques from Theorem~\ref{them:enum_explore} are applicable.
We note that since the Mazurkiewicz interleavings always have to be generated among sequential traces (i.e., straight-line programs),
we are generating them optimally (i.e., obtaining exactly one trace per Mazurkiewicz class) easily, using vector clocks~\cite{Mattern89}.
See Figure~\ref{fig:clyclic_star} for an illustration.

\input{fig_cyclic_star}





\smallskip\noindent{\bf Optimizations.}
Since our focus is on demonstrating a new, data-centric principle of DPOR, we focused on a basic implementation and avoided engineering optimizations.
We outline two straightforward algorithmic optimizations which were simple and useful.
\begin{compactenum}
\item (\emph{Burst mutations}). 
Instead of performing one mutation at a time, the algorithm performs a sequence of several mutations at once.
In particular, given a trace $\Trace$, any time we want to add a pair $(\Read, \Write)$ to the positive annotation,
we also add $(\Read', \Obs_{\Trace}(\Read'))$, where $\Read'\in \Past_{\Trace}(\Read)\cup \Past_{\Trace}(\Write)$
ranges over all read events in the causal past of $\Read$ and $\Write$ in $\Trace$.
This makes the recursion tree shallower, as now we do not need to apply any mutation $(\Read, \Write)$, where $\Write=\Obs_{\Trace}(\Read)$, individually.
\item (\emph{Cycle detection}). As a preprocessing step, before executing procedure $\Realize$ on some positive annotation $\Annotationpos$ input,
we test whether the graph $G$ (in Line~\ref{line:graph_G}) already contains a cycle.
The existence of a cycle is a proof that $\Annotationpos$ is not realizable, and requires linear instead of cubic time, as the graph is sparse.
\end{compactenum}



\subsection{Experimental Results}\label{subsec:experiments}

We now turn our attention to the experimental results.
We note that the comparison is not with MCR~\cite{HUANG15}, since MCR is value-based, and thus lies in a different class of approaches, where 
Instead, the comparison is with the recently developed Source-DPOR~\cite{Abdulla14}, which is based on discovering traces by ordering read-write events,
in the standard setting of~\cite{Flanagan05}.

\smallskip\noindent{\bf Experimental setup.}
In our experiments, we have compared our data-centric DPOR, with the Mazurkiewicz-based Source-DPOR  introduced recently in~\cite{Abdulla14} as an important improvement over the traditional DPOR~\cite{Flanagan05}.
Our benchmark set consists of synthetic benchmarks, as well as benchmarks obtained from the TACAS Competition on Software Verification (SV-COMP).
Most of the benchmarks have tunable size, by specifying a loop-unroll bound, or the number of threads running in parallel.
In all cases, we compared th running time and number of traces explored by $\EnumExplore$ and Source-DPOR.
We have set a timeout of 1 hour.
All benchmarks were executed on an Ubuntu-based virtual machine, given 4GB of memory and one 2GHz CPU.

\smallskip\noindent{\bf Two synthetic benchmarks.}
First we analyze the two synthetic benchmarks \emph{lastzero} and \emph{opt\_lock}, found in Table~\ref{tab:experiments_lastzero} and Table~\ref{tab:experiments_optlock} respectively.
The benchmark \emph{lastzero} was introduced in~\cite{Abdulla14} to demonstrate the superiority of Source-DPOR over the traditional DPOR from~\cite{Flanagan05}.
It consists of $n$ threads writing to an array, and $1$ thread reading from it (pseudocode in Appendix Section~\ref{sec:benchmarks}).
We observe that our $\EnumExplore$ explores exponentially fewer traces than Source-DPOR.
In fact, the number of traces explored by  our data-centric approach scales polynomially, whereas the number explored by the Mazurkiewicz-based approach grows exponentially with the number of threads.
Consequently, our $\EnumExplore$ runs much faster, and manages to scale on larger input sizes.
We note that the number of traces explored from Source-DPOR differs from the number reported in~\cite{Abdulla14}.
This is natural as the implementation of~\cite{Abdulla14} handles programs written in Erlang, a functional language with concurrency mechanisms much different from C.

The benchmark \emph{\emph{opt\_lock}} mimics an optimistic locking scheme of 2 threads (pseudocode in Appendix Section~\ref{sec:benchmarks}).
Each thread tries to update some variable, and afterwards checks if it was interrupted.
If not, it terminates, otherwise it tries again, up to a total $n$ number of attempts.
Again, we see that the number of explored traces by $\EnumExplore$ grows polynomially, whereas 
the number explored by Source-DPOR grows exponentially. 
Hence, our algorithm manages to handle much larger input sizes than the Mazurkiewicz-based Source-DPOR.
Recall that, as Theorem~\ref{them:enum_explore} states, this exponential reduction in the explored traces comes with polynomial-time guarantees per trace.


\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushleft}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
lastzero(4) & 38  & 2,118 & 0.21 & 0.84\\
\hline
lastzero(5) & 113 & 53,172 & 0.34 & 19.29\\ 
\hline
lastzero(6) &  316 & 1,765,876 & 0.63 & 856 \\
\hline
lastzero(7) & 937 & \footnotesize{-} & 1.8 & \footnotesize{-}\\
\hline
lastzero(8) & 3,151 & \footnotesize{-} & 9.32 &  \footnotesize{-}\\
\hline
lastzero(9) & 12,190 & \footnotesize{-} & 47.97 & \footnotesize{-}\\
\hline
lastzero(10) & 52,841  & \footnotesize{-} & 383.12 &\footnotesize{-}\\
%\hline
%lastzero(11) & 247,733 & \footnotesize{-} & 5,652.53 & \footnotesize{-}\\
\hline
\end{tabular}
\caption{Experiments on lastzero($n$), for $n+1$ threads.
'-' indicates a timeout after 1 hour.}
\label{tab:experiments_lastzero}
\end{table}
\end{flushleft}
\end{minipage}
\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushright}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
%opt\_lock(6) & 69  &2,442  & 0.22 & 0.82\\
%\hline
%opt\_lock(7) & 81 & 6,390  & 0.26 & 1.86 \\
%\hline
%opt\_lock(8) & 93 & 16,726 & 0.27 &4.95 \\
%\hline
%opt\_lock(9) & 105 & 43,786  & 0.27 & 13.07  \\
%\hline
%opt\_lock(10) & 117  & 114,630 & 0.31  &34.21   \\
%\hline
%opt\_lock(11) & 129 & 300,102 & 0.31  &  98.75 \\
%\hline
opt\_lock(12) & 141 & 785,674 & 0.35 &  252.64 \\
\hline
opt\_lock(13) & 153 & 2,056,918 & 0.36 &  703.90 \\
\hline
opt\_lock(14) & 165 & 5,385,078  & 0.43    & 18,80.12 \\
\hline
opt\_lock(15) & 177 & \footnotesize{-}  & 0.46   & \footnotesize{-} \\
\hline
opt\_lock(50) & 597 & \footnotesize{-} & 5.91 & \footnotesize{-}\\
\hline
opt\_lock(100) & 1,197 & \footnotesize{-} & 43.82 & \footnotesize{-}\\
\hline
opt\_lock(200) & 2,397 & \footnotesize{-} & 450.99 & \footnotesize{-}\\
\hline
\end{tabular}
\caption{Experiments on opt\_lock($n$), where $n$ is the number of attempts to optimistically lock.
'-' indicates a timeout after 1 hour.}
\label{tab:experiments_optlock}
\end{table}
\end{flushright}
\end{minipage}


\smallskip\noindent{\bf Benchmarks from SV-COMP.}
We now turn our attention to benchmarks from SV-COMP, namely 
\emph{fib\_bench}, \emph{pthread\_demo}, \emph{sigma\_false} and \emph{parker},
which are found in Table~\ref{tab:experiments_fib_bench}, Table~\ref{tab:experiments_pthread}, Table~\ref{tab:experiments_sigma}, and Table~\ref{tab:experiments_parker} respectively.
Similarly to our findings on the synthetic benchmarks, the data-centric $\EnumExplore$ manages to explore fewer traces than the Mazurkiewicz-based Source-DPOR.
In almost all cases, our algorithm run much faster, offering exponential gains in terms of time.
One exception is the benchmark \emph{parker}, where our $\EnumExplore$ is slower.
Although the number of traces explored is less than that of Source-DPOR,
the latter method managed to spend less time in discovering each trace, which led to a smaller overall time.
We note, however, that the improvement of Source-DPOR over $\EnumExplore$ appears to grow only as a small polynomial wrt the input size.
Recall that new traces are discovered by $\EnumExplore$ using the procedure $\Realize$, which can take cubic time in the worst case (Theorem~\ref{them:annotation}).
Hence, we identify optimizations to $\Realize$ as an important challenge that will contribute further to the scalability of our approach.


\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushleft}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
fib\_bench(4) & 1,233 & 19,605 & 0.93  & 3.03 \\
\hline
fib\_bench(5) & 8,897 & 218,243 & 7.41 & 37.82 \\
\hline
fib\_bench(6) & 70,765  & 2,364,418  & 85.71  & 463.52 \\
\hline
\end{tabular}
\caption{Experiments on fib\_bench($n$), where $n$ is the loop-unroll bound.}
\label{tab:experiments_fib_bench}
\end{table}
\end{flushleft}
\end{minipage}
\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushright}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
pthread\_demo(8) & 256 & 12,870 & 0.37 & 3.17 \\
\hline
pthread\_demo(10) & 1,024 & 184,756 & 1.23 & 49.51 \\
\hline
pthread\_demo(12) & 4,096 & 2,704,156 & 5.30 & 884.99 \\
\hline
\end{tabular}
\caption{Experiments on pthread\_demo($n$), where $n$ is the loop-unroll bound.}
\label{tab:experiments_pthread}
\end{table}
\end{flushright}
\end{minipage}





\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushleft}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
sigma\_false(6) & 16 & 10,395 & 0.22 & 2.57 \\
\hline
sigma\_false(7) & 22 & 135,135 &  0.26 & 38.41 \\
\hline
sigma\_false(8) & 29 & 2,027,025 & 0.28 & 658.27 \\
\hline
sigma\_false(9) & 37 & - & 0.38 & - \\
\hline
sigma\_false(10) & 46 & - & 0.44 & -\\
\hline
\end{tabular}
\caption{Experiments on sigma\_false($n$), where $n$ is the loop-unroll bound.
'-' indicates a timeout after 1 hour.}
\label{tab:experiments_sigma}
\end{table}
\end{flushleft}
\end{minipage}
\qquad
\begin{minipage}[t]{.49\textwidth}
\vspace{0pt}
\begin{flushright}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{1pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
parker(8) & 1,254 & 3,343 & 1.52 & 1.33 \\
\hline
parker(10) & 2,411 & 6,212 & 5.03 & 3.96\\
\hline
parker(12) & 4,132 & 10,361 & 8.09  & 5.62\\
\hline
parker(14) & 6,529 & 16,022  & 11.96  & 6.86\\
\hline
parker(16) & 9,714 & 23,427  & 19.89  & 10.85\\
\hline
\end{tabular}
\caption{Experiments on parker($n$), where $n$ is the loop-unroll bound.}
\label{tab:experiments_parker}
\end{table}
\end{flushright}
\end{minipage}


\begin{comment}
\begin{table}[H]
\footnotesize
\setlength\tabcolsep{2pt}
\begin{tabular}{|c||c c|c c|}
\hline
\textbf{Benchmark} & \multicolumn{2}{c|}{\textbf{Traces}} & \multicolumn{2}{c|}{\textbf{Time (s)}}\\
\hline
& DC-DPOR  & S-DPOR & DC-DPOR  & S-DPOR \\
\hline
\hline
fib\_bench(4) & 1,233 & 19,605 & 0.93  & 3.03 \\
\hline
fib\_bench(5) & 8,897 & 218,243 & 7.41 & 37.82 \\
\hline
fib\_bench(6) & 70,765  & 2,364,418  & 85.71  & 463.52 \\
\hline
scull\_true & 58 & 5,602  & 0.5 & 3.84\\
\hline
dekker & 35  & 64   & 0.20  & 0.14 \\
\hline
lamport & 13 & 32  & 0.17  & 0.15\\
\hline
parker(8) & 1,254 & 3,343 & 1.52 & 1.33 \\
\hline
parker(10) & 2,411 & 6,212 & 5.03 & 3.96\\
\hline
parker(12) & 4,132 & 10,361 & 8.09  & 5.62\\
\hline
parker(14) & 6,529 & 16,022  & 14.33 & 8.79\\
\hline
peterson & 10 & 10 & 0.13 & 0.14\\
\hline
peterson\_trial & 23,052 & 31,200 &18.68 & 5.86\\
\hline
pgsql(100) &  3 & 400 & 1.00 & 0.51 \\
\hline
pgsql(150) &  3 & 400 & 2.54 & 0.94 \\
\hline
pgsql(200) &  3 & 400 & 6.48 & 1.53 \\
\hline
pgsql\_bnd(3) & 245 & 364 & 0.33 & 0.31\\
\hline
pgsql\_bnd(4) & 16,386  &  21,845  & 9.52 & 8.1\\
\hline
pgsql\_bnd(5) & 279,938  &  335,923  & 217.88 & 99.28\\
\hline
pthread\_demo(7) & 128 & 3,432 & 0.30 & 1.2\\
\hline
pthread\_demo(8) & 256 & 12,870 & 0.37 & 3.17 \\
\hline
pthread\_demo(9) & 512 & 48,620 & 0.61 & 14.82 \\
\hline
pthread\_demo(10) & 1,024 & 184,756 & 1.23 & 49.51 \\
\hline
pthread\_demo(11) & 2,048 & 705,432 & 2.27 & 204.72 \\
\hline
pthread\_demo(12) & 4,096 & 2,704,156 & 5.30 & 884.99 \\
\hline
pthread\_demo(13) & 8,192 & - & 10.99 & - \\
\hline
pthread\_demo(14) & 16,384 & - & 25.35 & -\\
\hline
pthread\_demo(15) & 32,768 & - & 54.01 & -\\
\hline
sigma\_false(6) & 16 & 10,395 & 0.22 & 2.57 \\
\hline
sigma\_false(7) & 22 & 135,135   0.26& & 38.41 \\
\hline
sigma\_false(8) & 29 & 2,027,025 & 0.28 & 658.27 \\
\hline
sigma\_false(9) & 37 & - & 0.38 & - \\
\hline
sigma\_false(10) & 46 & - & 0.44 & -\\
\hline
sigma\_false(15) & 106 & 0 & 2.79 & - \\
\hline
stack\_safe(4) & 152 &  & 0.42 & 0.39 \\
\hline
stack\_safe(5) & 548 & 1005 & 1.39 & 0.78\\
\hline
\hline
\end{tabular}
\caption{}
\label{tab:experiments_fib}
\end{table}
\end{comment}

==> experiments_old.tex <==
\section{Experiments}\label{sec:experiments}
%\vspace{-0.5em}

%%In this e current section 
We report on a basic experimental evaluation of our data-centric DPOR,
and compare it to the standard DPOR of~\cite{Flanagan05}.
We refer to Appendix~\cref{sec:benchmarks} for further details on experiments,
and the set of benchmarks used.
%Since that method has no upper-bound on the number of representative traces explored from each Mazurkiewicz class,
%we also report on the number of Mazurkiewicz classes in each case.

%
\noindent{\bf Experimental setup.}
We have implemented our $\EnumExplore$ algorithm in Python, and evaluate its performance on a set of academic benchmarks.
Our basis for comparison is also a Python implementation of~\cite[Figure~4]{Flanagan05}.
All benchmarks are straightforwardly translated to our model.
The experiments were run on a standard desktop computer with 3.5GHz CPU.



%
\noindent{\bf Results.}
We report the results of our evaluation in \cref{tab:results}.
Each section of the table starts with the benchmark name, the parameter that was used in order to obtain the results for the specific benchmark (e.g., number loop iterations, number of threads) and the time bound that was used for timeouts.
We varied the timeout bound in order to obtain enough points for a comparison.
Timeout cases are reported with ``-''.
The first column reports the parameter values that were used to obtain the respective row.
The values of the corresponding table columns were calculated as follows.
\begin{compactenum}
\item $|\sim_{M}|$ reports an underapproximation of number of Mazurkiewicz classes, wrt \emph{not necessarily maximal} traces.
See Appendix~\cref{sec:benchmarks} for details on this underapproximation.
\item DC-DPOR~(\#~$\Annotationpos$) reports the number of positive annotations (i.e., observation classes, not necessarily maximal) explored by DC-DPOR.
\item DPOR~(s) and DC-DPOR~(s) report the running time (in seconds) of the corresponding method.
\end{compactenum}
We see that running times scale better in our DC-DPOR than the standard DPOR.
Additionally, the number of observation classes examined by DC-DPOR scales better than (the underapproximation of ) $|\sim_{M}|$.


\begin{table}
\centering
\footnotesize
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{1pt}
\begin{tabular}{c||c|c|c|c}
{\normalsize \bf \#}& {\normalsize \bf $\mathbf{|\sim_{M}|}$}  & {\normalsize \bf DC-DPOR (\# $\Annotationpos$)} & {\normalsize \bf DPOR (s)}  & {\normalsize \bf DC-DPOR (s)}\\
\hline
\hline
\hline
\multicolumn{5}{c}{(2~Processes)~~\textbf{Alternate write-read}~$(n)$~~$\mathsf{TO}=5\mathsf{h}$}\\
\hline
\hline
%1 & 4 & 4 & 3 & 0.01 & 0.00\\
%\hline
%2 & 34  & 46 & 19 & 0.11 & 0.03\\
%\hline
%3 & 328  & 610 & 141 & 1.2 & 0.3\\
%\hline
(4) & 8335  & 1107 & 19 & 5\\
\hline
(5) & 87260 & 8953 & 327 & 63\\
\hline
(6) & 931090 & 73789 & 5514 & 790\\
\hline
(7) & - & 616227 & - & 10015\\
\hline
\multicolumn{5}{c}{($k$~Processes)~~\textbf{Pipeline}~$(k)$~~$\mathsf{TO}=4\mathsf{h}$}\\
\hline
\hline
(9) & 163840 & 6561 & 816 & 43\\
\hline
(10) & 655360  & 19683 & 3170 & 156\\
\hline
(11) & 2621440 & 59049 & 14561 & 544\\
\hline
(12) & - & 177147 & - & 1893\\
\hline
(13) & - & 531441 & - & 6520\\
\hline
\multicolumn{5}{c}{(2~Processes)~~\textbf{Commits}~$(c)$~~$\mathsf{TO}=6\mathsf{h}$}\\
\hline
\hline
%1 & 8 & 10 & 7 & 0.12 & 0.02\\
%\hline
(2) & 1060  & 293 & 10.7 & 1.8\\
\hline
(3) & 77830 & 16401 & 1977 & 216\\
\hline
(4) & - & 1008755 & - & 23768\\
\hline
\multicolumn{5}{c}{(2~Processes)~~\textbf{Eratosthenes}~$(N)$~~$\mathsf{TO}=12\mathsf{h}$}\\
\hline
\hline
%a & 4.0 & 3.0 & 0.0934829711914 & 0.00825095176697\\
%\hline
%a & 16.0 & 11.0 & 0.644221067429 & 0.0439839363098\\
%\hline
%a & 34.0 & 28.0 & 3.20801591873 & 0.258011102676\\
%\hline
%(4) & 340 & 98 & 37 & 0.9\\
%\hline
(5) & 995 & 305 & 550 & 8\\
\hline
(6) & 3980 & 1045 & 6697 & 26\\
\hline
(7) & 6720 & 2840 & 34849 & 173\\
\hline
(8) & - & 4333 & - & 444\\
\hline
\multicolumn{5}{c}{(2~Processes)~~\textbf{Peterson}~$(c,a)$~~$\mathsf{TO}=5\mathsf{h}$}\\
\hline
\hline
%a & 18.0 & 20.0 & 0.816300153732 & 0.099189043045\\
\hline
(1,2) & 145 & 90 & 7 & 0.6\\
\hline
(1,3) & 275 & 222 & 32 & 2\\
\hline
(2,1) & 2795 & 1499 & 1096 & 18\\
\hline
(2,2) & - & 26110 & - & 649\\
\hline
(2,3) & - & 155419 & - & 7240\\
\hline
(3,1) & - & 117916 & - & 3593\\
\hline
\multicolumn{5}{c}{(2~Processes)~~\textbf{KeyRotation}~~$(c)$~~$\mathsf{TO}=4\mathsf{h}$}\\
\hline
\hline
%(1) & 8.0 & 7.0 & 0.0494577884674 & 0.014848947525\\
%\hline
(2) & 570 & 181 & 6 & 0.9\\
\hline
(3) & 18620 & 5503 & 1757 & 65\\
\hline
(4) & - & 176503 & - & 4291\\
\hline
%\multicolumn{5}{c}{\textbf{LastZero}~$(k)$~~$\mathsf{TO}=6\mathsf{h}$}
%\hline
%\hline
%(3) & 12 & 5 & 0.6 & 0.03\\
%\hline
%(4) & 40 & 21 & 65 & 0.4\\
%\hline
%(5) & 105 & 103 & 18057 & 4\\
%\hline
%(6) & - & 657 & - & 69\\
%\hline
%(7) & - & 4837 & - & 998\\
%\hline
%(8) & - & 40117 & - & 15260\\
%\hline
\end{tabular}
\caption{Experimental evaluation and comparison to~\cite{Flanagan05}.}
\label{tab:results}
\end{table}




\begin{comment}
\begin{table}
\small
\renewcommand{\arraystretch}{1}
\setlength\tabcolsep{3pt}
\begin{tabular}{c||c|c|c|c|c}
{\bf \#}& {\bf $\mathbf{|\sim_{M}|}$}  & {\bf DPOR (t)}  & {\bf DC-DPOR (t)} & {\bf DPOR (s)}  & {\bf DC-DPOR (s)}\\
\hline
\hline
\hline
\multicolumn{6}{c}{\textbf{Alternate write-read}~$(n)$~~$\mathsf{TO}=$}\\
\hline
\hline
%1 & 4 & 4 & 3 & 0.01 & 0.00\\
%\hline
%2 & 34  & 46 & 19 & 0.11 & 0.03\\
%\hline
%3 & 328  & 610 & 141 & 1.2 & 0.3\\
%\hline
(4) & 3334 & 8518 & 1107 & 19 & 5\\
\hline
(5) & 34904 & 122464 & 8953 & 327 & 63\\
\hline
(6) & 372436 & 1794196 & 73789 & 5514 & 790\\
\hline
(7) & - & - & 616227 & - & 10015\\
\hline
\multicolumn{6}{c}{\textbf{Pipeline}~$(n)$~~$\mathsf{TO}=4\mathsf{h}$}\\
\hline
\hline
(9) & 65536 & 65536 & 6561 & 816 & 43\\
\hline
(10) & 262144 & 262144 & 19683 & 3170 & 156\\
\hline
(11) & 1048576 & 1048576 & 59049 & 14561 & 544\\
\hline
(12) & - & - & 177147 & - & 1893\\
\hline
(13) & - & - & 531441 & - & 6520\\
\hline
\multicolumn{6}{c}{\textbf{Commits}~$(c)$~~$\mathsf{TO}=6\mathsf{h}$}\\
\hline
\hline
%1 & 8 & 10 & 7 & 0.12 & 0.02\\
%\hline
(2) & 424 & 1003 & 293 & 10.7 & 1.8\\
\hline
(3) & 31132 & 140101 & 16401 & 1977 & 216\\
\hline
(4) & - & - & 1008755 & - & 23768\\
\hline
\multicolumn{6}{c}{\textbf{Peterson}~$(c,a)$~~$\mathsf{TO}=8\mathsf{h}$}\\
\hline
\hline
%1 & 18 & 146 & 20 & 0.81 & 0.09\\
\hline
2 & 58 & 1066 & 90 & 7 & 0.6\\
\hline
3 & 110 & 4029 & 222 & 32 & 2\\
\hline
4 & 1118 & 111768 & 1499 & 1096 & 19\\
\hline
5 & - & - & 26110 & - & 932\\
\hline
6 & - & - & 117916 & - & 5831\\
\hline
7 & - & - & 155419 & - & 11301\\
\hline
\multicolumn{6}{c}{\textbf{LastZero}}\\
\hline
\hline
\hline
\end{tabular}
\caption{Experimental comparison of $\EnumExplore$ to~\cite{Flanagan05}.}
\label{tab:results}
\end{table}

\end{comment}

==> guided.tex <==
\section{Search Pruning}\label{sec:guided}

{\bf AP: Add example}

As we have already seen in \cref{sec:mazurkiewicz}, our data-centric DPOR search is guaranteed to explore fewer traces that any DPOR search based on Mazurkiewicz traces. 
In this section we highlight an important feature of our algorithm that can be used to guide the bug search towards faster bug finding,
or dynamically prune away parts of the trace space that are guaranteed to not lead in bug manifestation (e.g., to an assertion violation).

\smallskip\noindent{\bf Monotonicity of annotations.}
Consider the recursion tree $\RecTree$ of our data-centric DPOR, and for each node $u$, denote by $\Trace_u$ and $\Annotation_u=(\Annotationpos_u, \Annotationneg_u)$ the trace and annotation input of the algorithm on that node.
For every read event $\Read\in\Annotationpos_u$, every other read event in the observable past cone of $\Read$ is also in $\Annotationpos_u$.
Additionally, the algorithm never relaxes annotations (i.e., it never removes an annotated read from $\Annotationpos$,
hence the annotations are only strengthened along each path from the root of $\RecTree$ to each of its leaves.
The consequences of this monotonicity property is stated in the following remark.

\smallskip
\begin{remark}[Monotonicity of annotations]\label{rem:monotonicity}
For every node $u$ of $\RecTree$ and descendant $v$ of $u$, for every read $\Read\in\Domain(\Annotationpos_u)$ we have that
$\Read\in\Domain(\Annotationpos_v)$ and $\Value_{\Trace_u}(\Read)=\Value_{\Trace_v}(\Read)$.
\end{remark}

\cref{rem:monotonicity} states particularly useful feature that can be exploited dynamically to guide the search, in order to explore fewer classes of $\TraceSpace/\sim_{\Obs}$ in the process of bug discovery.
This speedup can arise in form of \emph{search pruning}.
For ease of presentation, we assume that we are interested in detecting a particular assertion violation event.
That is, we focus on a single read event $\Read$ of a target process $\Process_i$.
The event $\Read$ is associated with the assertion, and we are interested in detecting whether there exists a trace $\Trace$ such that $\Read\in\Events{\Trace}$ and $\Value_{\Trace}(\Read)=\False$ (i.e., the assertion fails in $\Trace$).
We call such a trace a \emph{buggy trace}.


\smallskip\noindent{\bf Search pruning.}
In search pruning, the algorithm will prune away subtrees $\RecTree_u$ of the recursion tree $\RecTree$ rooted on specific nodes $u$ when $\RecTree_u$ is guaranteed to not explore any buggy traces.
This is holds in the following cases.
\begin{compactenum}
\item\label{item:prune_value} If $\Read\in\Domain(\Annotationpos_u)$ and $\Trace_u$ is not a failing trace, since every trace $\Trace_v$ of each node $v$ in $\RecTree_u$ agrees with $\Trace_u$ on the value of $\Read$, $\Trace_v$ is guaranteed to not be a buggy trace.
\item\label{item:prune_enable} Let $\Read_i$ be the last read event of the target process $\Process_i$ in $\Annotationpos_u$.
If $\Read_i$ is not ordered before $\Read$ by the program structure, i.e., it is not the case that $\PS(\Read_i,\Read)$,
then $\Read$ is guaranteed to not appear in any trace $\Trace_v$ of a node $v$ that belongs to $\RecTree_u$,
hence no such $\Trace_v$ is a buggy trace.
\item\label{item:prune_invariant} There exists a rich body of work~\cite{Shi10,Wang11,Gupta15,} which attempts to learn sets of good traces, i.e., sets that contain traces that do not manifest erroneous behavior.
Often such sets are characterized by observation functions, i.e., all traces in a good set agree on certain properties of their observation functions.
As an example, we focus on the work of~\cite{Wang11}.
The authors introduce the so-called \emph{definition-use invariants}, which are intended invariants on the observations of specific read events in the program. For instance, a \emph{local invariant} on a read event $\Read$ states that in every trace $\Trace$,
$\Read$ and $\Obs_{\Trace}(\Read)$ must belong to the same process (i.e., $\Read$ observes a local write),
whereas a \emph{remote invariant} states that $\Read$ and $\Obs_{\Trace}(\Read)$ must belong to different processes.
Such invariants can either be supplied by the programmer, or automatically inferred by some learning algorithm~\cite{Wang11}.
Given a guarantee that a trace which satisfies all intended invariants is not a buggy trace,
if the search encounters a node $u$ where the positive annotation $\Annotationpos_u$ satisfies all such invariants, the search can prune away $\RecTree_u$, as any trace $\Trace_v$ of each node $v$ of $\RecTree_u$ is guaranteed to satisfy those invariants as well.
\end{compactenum}


\begin{comment}
\smallskip\noindent{\bf Search guiding.}
In search guiding, given a node $u$, the algorithm will choose to explore the children $u_1,\dots,u_n$ of $u$ in some specific order, based on the likelihood that each child $u_i$ contains a buggy trace in its subtree $\RecTree_{u_i}$.
The idea is similar to \cref{item:prune_invariant} of search pruning, where now guarantees on the goodness of annotations is replaced by beliefs on how likely it is for each annotation $\Annotationpos_{v_i}$ to have a compatible trace in the subtree $\RecTree_{v_i}$ which is also buggy.
There exist several approaches that make this kind of estimates~\cite{Farzan09,Shi10,Sorrentino10,Wang11,Razavi11,Zeng12,Farzan12}.



Note that search pruning and search guiding are orthogonal to each other, and can be used in combination.
To our knowledge, the traditional control-centric DPOR algorithms based on Mazurkiewicz traces do not enjoy such monotonicity properties,
and hence it is unclear whether guiding the search is possible (or easy).
\end{comment}
